Evidence for the Higgs boson decay to a $Z$ boson and a photon at the LHC

The first evidence for the Higgs boson decay to a $Z$ boson and a photon is presented, with a statistical significance of 3.4 standard deviations. The result is derived from a combined analysis of the searches performed by the ATLAS and CMS Collaborations with proton-proton collision data sets collected at the CERN Large Hadron Collider (LHC) from 2015 to 2018. These correspond to integrated luminosities of around 140 fb$^{-1}$ for each experiment, at a center-of-mass energy of 13 TeV. The measured signal yield is $2.2\pm0.7$ times the Standard Model prediction, and agrees with the theoretical expectation within 1.9 standard deviations.

==> cms-authorlist.tex <==

\cmsinstitute{Yerevan Physics Institute, Yerevan, Armenia}
{\tolerance=6000
A.~Hayrapetyan, A.~Tumasyan\cmsAuthorMark{1}\cmsorcid{0009-0000-0684-6742}
\par}
\cmsinstitute{Institut f\"{u}r Hochenergiephysik, Vienna, Austria}
{\tolerance=6000
W.~Adam\cmsorcid{0000-0001-9099-4341}, J.W.~Andrejkovic, T.~Bergauer\cmsorcid{0000-0002-5786-0293}, S.~Chatterjee\cmsorcid{0000-0003-2660-0349}, K.~Damanakis\cmsorcid{0000-0001-5389-2872}, M.~Dragicevic\cmsorcid{0000-0003-1967-6783}, A.~Escalante~Del~Valle\cmsorcid{0000-0002-9702-6359}, P.S.~Hussain\cmsorcid{0000-0002-4825-5278}, M.~Jeitler\cmsAuthorMark{2}\cmsorcid{0000-0002-5141-9560}, N.~Krammer\cmsorcid{0000-0002-0548-0985}, A.~Li\cmsorcid{0000-0002-4547-116X}, D.~Liko\cmsorcid{0000-0002-3380-473X}, I.~Mikulec\cmsorcid{0000-0003-0385-2746}, J.~Schieck\cmsAuthorMark{2}\cmsorcid{0000-0002-1058-8093}, R.~Sch\"{o}fbeck\cmsorcid{0000-0002-2332-8784}, D.~Schwarz\cmsorcid{0000-0002-3821-7331}, M.~Sonawane\cmsorcid{0000-0003-0510-7010}, S.~Templ\cmsorcid{0000-0003-3137-5692}, W.~Waltenberger\cmsorcid{0000-0002-6215-7228}, C.-E.~Wulz\cmsAuthorMark{2}\cmsorcid{0000-0001-9226-5812}
\par}
\cmsinstitute{Universiteit Antwerpen, Antwerpen, Belgium}
{\tolerance=6000
M.R.~Darwish\cmsAuthorMark{3}\cmsorcid{0000-0003-2894-2377}, T.~Janssen\cmsorcid{0000-0002-3998-4081}, P.~Van~Mechelen\cmsorcid{0000-0002-8731-9051}
\par}
\cmsinstitute{Vrije Universiteit Brussel, Brussel, Belgium}
{\tolerance=6000
E.S.~Bols\cmsorcid{0000-0002-8564-8732}, J.~D'Hondt\cmsorcid{0000-0002-9598-6241}, S.~Dansana\cmsorcid{0000-0002-7752-7471}, A.~De~Moor\cmsorcid{0000-0001-5964-1935}, M.~Delcourt\cmsorcid{0000-0001-8206-1787}, H.~El~Faham\cmsorcid{0000-0001-8894-2390}, S.~Lowette\cmsorcid{0000-0003-3984-9987}, I.~Makarenko\cmsorcid{0000-0002-8553-4508}, D.~M\"{u}ller\cmsorcid{0000-0002-1752-4527}, A.R.~Sahasransu\cmsorcid{0000-0003-1505-1743}, S.~Tavernier\cmsorcid{0000-0002-6792-9522}, M.~Tytgat\cmsAuthorMark{4}\cmsorcid{0000-0002-3990-2074}, S.~Van~Putte\cmsorcid{0000-0003-1559-3606}, D.~Vannerom\cmsorcid{0000-0002-2747-5095}
\par}
\cmsinstitute{Universit\'{e} Libre de Bruxelles, Bruxelles, Belgium}
{\tolerance=6000
B.~Clerbaux\cmsorcid{0000-0001-8547-8211}, G.~De~Lentdecker\cmsorcid{0000-0001-5124-7693}, L.~Favart\cmsorcid{0000-0003-1645-7454}, D.~Hohov\cmsorcid{0000-0002-4760-1597}, J.~Jaramillo\cmsorcid{0000-0003-3885-6608}, A.~Khalilzadeh, K.~Lee\cmsorcid{0000-0003-0808-4184}, M.~Mahdavikhorrami\cmsorcid{0000-0002-8265-3595}, A.~Malara\cmsorcid{0000-0001-8645-9282}, S.~Paredes\cmsorcid{0000-0001-8487-9603}, L.~P\'{e}tr\'{e}\cmsorcid{0009-0000-7979-5771}, N.~Postiau, L.~Thomas\cmsorcid{0000-0002-2756-3853}, M.~Vanden~Bemden\cmsorcid{0009-0000-7725-7945}, C.~Vander~Velde\cmsorcid{0000-0003-3392-7294}, P.~Vanlaer\cmsorcid{0000-0002-7931-4496}
\par}
\cmsinstitute{Ghent University, Ghent, Belgium}
{\tolerance=6000
M.~De~Coen\cmsorcid{0000-0002-5854-7442}, D.~Dobur\cmsorcid{0000-0003-0012-4866}, Y.~Hong\cmsorcid{0000-0003-4752-2458}, J.~Knolle\cmsorcid{0000-0002-4781-5704}, L.~Lambrecht\cmsorcid{0000-0001-9108-1560}, G.~Mestdach, C.~Rend\'{o}n, A.~Samalan, K.~Skovpen\cmsorcid{0000-0002-1160-0621}, N.~Van~Den~Bossche\cmsorcid{0000-0003-2973-4991}, L.~Wezenbeek\cmsorcid{0000-0001-6952-891X}
\par}
\cmsinstitute{Universit\'{e} Catholique de Louvain, Louvain-la-Neuve, Belgium}
{\tolerance=6000
A.~Benecke\cmsorcid{0000-0003-0252-3609}, G.~Bruno\cmsorcid{0000-0001-8857-8197}, C.~Caputo\cmsorcid{0000-0001-7522-4808}, C.~Delaere\cmsorcid{0000-0001-8707-6021}, I.S.~Donertas\cmsorcid{0000-0001-7485-412X}, A.~Giammanco\cmsorcid{0000-0001-9640-8294}, K.~Jaffel\cmsorcid{0000-0001-7419-4248}, Sa.~Jain\cmsorcid{0000-0001-5078-3689}, V.~Lemaitre, J.~Lidrych\cmsorcid{0000-0003-1439-0196}, P.~Mastrapasqua\cmsorcid{0000-0002-2043-2367}, K.~Mondal\cmsorcid{0000-0001-5967-1245}, T.T.~Tran\cmsorcid{0000-0003-3060-350X}, S.~Wertz\cmsorcid{0000-0002-8645-3670}
\par}
\cmsinstitute{Centro Brasileiro de Pesquisas Fisicas, Rio de Janeiro, Brazil}
{\tolerance=6000
G.A.~Alves\cmsorcid{0000-0002-8369-1446}, E.~Coelho\cmsorcid{0000-0001-6114-9907}, C.~Hensel\cmsorcid{0000-0001-8874-7624}, T.~Menezes~De~Oliveira, A.~Moraes\cmsorcid{0000-0002-5157-5686}, P.~Rebello~Teles\cmsorcid{0000-0001-9029-8506}, M.~Soeiro
\par}
\cmsinstitute{Universidade do Estado do Rio de Janeiro, Rio de Janeiro, Brazil}
{\tolerance=6000
W.L.~Ald\'{a}~J\'{u}nior\cmsorcid{0000-0001-5855-9817}, M.~Alves~Gallo~Pereira\cmsorcid{0000-0003-4296-7028}, M.~Barroso~Ferreira~Filho\cmsorcid{0000-0003-3904-0571}, H.~Brandao~Malbouisson\cmsorcid{0000-0002-1326-318X}, W.~Carvalho\cmsorcid{0000-0003-0738-6615}, J.~Chinellato\cmsAuthorMark{5}, E.M.~Da~Costa\cmsorcid{0000-0002-5016-6434}, G.G.~Da~Silveira\cmsAuthorMark{6}\cmsorcid{0000-0003-3514-7056}, D.~De~Jesus~Damiao\cmsorcid{0000-0002-3769-1680}, S.~Fonseca~De~Souza\cmsorcid{0000-0001-7830-0837}, J.~Martins\cmsAuthorMark{7}\cmsorcid{0000-0002-2120-2782}, C.~Mora~Herrera\cmsorcid{0000-0003-3915-3170}, K.~Mota~Amarilo\cmsorcid{0000-0003-1707-3348}, L.~Mundim\cmsorcid{0000-0001-9964-7805}, H.~Nogima\cmsorcid{0000-0001-7705-1066}, A.~Santoro\cmsorcid{0000-0002-0568-665X}, A.~Sznajder\cmsorcid{0000-0001-6998-1108}, M.~Thiel\cmsorcid{0000-0001-7139-7963}, A.~Vilela~Pereira\cmsorcid{0000-0003-3177-4626}
\par}
\cmsinstitute{Universidade Estadual Paulista, Universidade Federal do ABC, S\~{a}o Paulo, Brazil}
{\tolerance=6000
C.A.~Bernardes\cmsAuthorMark{6}\cmsorcid{0000-0001-5790-9563}, L.~Calligaris\cmsorcid{0000-0002-9951-9448}, T.R.~Fernandez~Perez~Tomei\cmsorcid{0000-0002-1809-5226}, E.M.~Gregores\cmsorcid{0000-0003-0205-1672}, P.G.~Mercadante\cmsorcid{0000-0001-8333-4302}, S.F.~Novaes\cmsorcid{0000-0003-0471-8549}, B.~Orzari\cmsorcid{0000-0003-4232-4743}, Sandra~S.~Padula\cmsorcid{0000-0003-3071-0559}
\par}
\cmsinstitute{Institute for Nuclear Research and Nuclear Energy, Bulgarian Academy of Sciences, Sofia, Bulgaria}
{\tolerance=6000
A.~Aleksandrov\cmsorcid{0000-0001-6934-2541}, G.~Antchev\cmsorcid{0000-0003-3210-5037}, R.~Hadjiiska\cmsorcid{0000-0003-1824-1737}, P.~Iaydjiev\cmsorcid{0000-0001-6330-0607}, M.~Misheva\cmsorcid{0000-0003-4854-5301}, M.~Shopova\cmsorcid{0000-0001-6664-2493}, G.~Sultanov\cmsorcid{0000-0002-8030-3866}
\par}
\cmsinstitute{University of Sofia, Sofia, Bulgaria}
{\tolerance=6000
A.~Dimitrov\cmsorcid{0000-0003-2899-701X}, L.~Litov\cmsorcid{0000-0002-8511-6883}, B.~Pavlov\cmsorcid{0000-0003-3635-0646}, P.~Petkov\cmsorcid{0000-0002-0420-9480}, A.~Petrov\cmsorcid{0009-0003-8899-1514}, E.~Shumka\cmsorcid{0000-0002-0104-2574}
\par}
\cmsinstitute{Instituto De Alta Investigaci\'{o}n, Universidad de Tarapac\'{a}, Casilla 7 D, Arica, Chile}
{\tolerance=6000
S.~Keshri\cmsorcid{0000-0003-3280-2350}, S.~Thakur\cmsorcid{0000-0002-1647-0360}
\par}
\cmsinstitute{Beihang University, Beijing, China}
{\tolerance=6000
T.~Cheng\cmsorcid{0000-0003-2954-9315}, Q.~Guo, T.~Javaid\cmsorcid{0009-0007-2757-4054}, M.~Mittal\cmsorcid{0000-0002-6833-8521}, L.~Yuan\cmsorcid{0000-0002-6719-5397}
\par}
\cmsinstitute{Department of Physics, Tsinghua University, Beijing, China}
{\tolerance=6000
G.~Bauer\cmsAuthorMark{8}$^{, }$\cmsAuthorMark{9}, Z.~Hu\cmsorcid{0000-0001-8209-4343}, J.~Liu, K.~Yi\cmsAuthorMark{8}$^{, }$\cmsAuthorMark{10}\cmsorcid{0000-0002-2459-1824}
\par}
\cmsinstitute{Institute of High Energy Physics, Beijing, China}
{\tolerance=6000
G.M.~Chen\cmsAuthorMark{11}\cmsorcid{0000-0002-2629-5420}, H.S.~Chen\cmsAuthorMark{11}\cmsorcid{0000-0001-8672-8227}, M.~Chen\cmsAuthorMark{11}\cmsorcid{0000-0003-0489-9669}, F.~Iemmi\cmsorcid{0000-0001-5911-4051}, C.H.~Jiang, A.~Kapoor\cmsAuthorMark{12}\cmsorcid{0000-0002-1844-1504}, H.~Liao\cmsorcid{0000-0002-0124-6999}, Z.-A.~Liu\cmsAuthorMark{13}\cmsorcid{0000-0002-2896-1386}, F.~Monti\cmsorcid{0000-0001-5846-3655}, M.A.~Shahzad\cmsAuthorMark{11}, R.~Sharma\cmsAuthorMark{14}\cmsorcid{0000-0003-1181-1426}, J.N.~Song\cmsAuthorMark{13}, J.~Tao\cmsorcid{0000-0003-2006-3490}, C.~Wang\cmsAuthorMark{11}, J.~Wang\cmsorcid{0000-0002-3103-1083}, Z.~Wang\cmsAuthorMark{11}, H.~Zhang\cmsorcid{0000-0001-8843-5209}
\par}
\cmsinstitute{State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing, China}
{\tolerance=6000
A.~Agapitos\cmsorcid{0000-0002-8953-1232}, Y.~Ban\cmsorcid{0000-0002-1912-0374}, A.~Levin\cmsorcid{0000-0001-9565-4186}, C.~Li\cmsorcid{0000-0002-6339-8154}, Q.~Li\cmsorcid{0000-0002-8290-0517}, Y.~Mao, S.J.~Qian\cmsorcid{0000-0002-0630-481X}, X.~Sun\cmsorcid{0000-0003-4409-4574}, D.~Wang\cmsorcid{0000-0002-9013-1199}, H.~Yang, L.~Zhang\cmsorcid{0000-0001-7947-9007}, M.~Zhang, C.~Zhou\cmsorcid{0000-0001-5904-7258}
\par}
\cmsinstitute{Sun Yat-Sen University, Guangzhou, China}
{\tolerance=6000
Z.~You\cmsorcid{0000-0001-8324-3291}
\par}
\cmsinstitute{University of Science and Technology of China, Hefei, China}
{\tolerance=6000
N.~Lu\cmsorcid{0000-0002-2631-6770}
\par}
\cmsinstitute{Institute of Modern Physics and Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) - Fudan University, Shanghai, China}
{\tolerance=6000
X.~Gao\cmsAuthorMark{15}\cmsorcid{0000-0001-7205-2318}, D.~Leggat, H.~Okawa\cmsorcid{0000-0002-2548-6567}, Y.~Zhang\cmsorcid{0000-0002-4554-2554}
\par}
\cmsinstitute{Zhejiang University, Hangzhou, Zhejiang, China}
{\tolerance=6000
Z.~Lin\cmsorcid{0000-0003-1812-3474}, C.~Lu\cmsorcid{0000-0002-7421-0313}, M.~Xiao\cmsorcid{0000-0001-9628-9336}
\par}
\cmsinstitute{Universidad de Los Andes, Bogota, Colombia}
{\tolerance=6000
C.~Avila\cmsorcid{0000-0002-5610-2693}, D.A.~Barbosa~Trujillo, A.~Cabrera\cmsorcid{0000-0002-0486-6296}, C.~Florez\cmsorcid{0000-0002-3222-0249}, J.~Fraga\cmsorcid{0000-0002-5137-8543}, J.A.~Reyes~Vega
\par}
\cmsinstitute{Universidad de Antioquia, Medellin, Colombia}
{\tolerance=6000
J.~Mejia~Guisao\cmsorcid{0000-0002-1153-816X}, F.~Ramirez\cmsorcid{0000-0002-7178-0484}, M.~Rodriguez\cmsorcid{0000-0002-9480-213X}, J.D.~Ruiz~Alvarez\cmsorcid{0000-0002-3306-0363}
\par}
\cmsinstitute{University of Split, Faculty of Electrical Engineering, Mechanical Engineering and Naval Architecture, Split, Croatia}
{\tolerance=6000
D.~Giljanovic\cmsorcid{0009-0005-6792-6881}, N.~Godinovic\cmsorcid{0000-0002-4674-9450}, D.~Lelas\cmsorcid{0000-0002-8269-5760}, A.~Sculac\cmsorcid{0000-0001-7938-7559}
\par}
\cmsinstitute{University of Split, Faculty of Science, Split, Croatia}
{\tolerance=6000
M.~Kovac\cmsorcid{0000-0002-2391-4599}, T.~Sculac\cmsorcid{0000-0002-9578-4105}
\par}
\cmsinstitute{Institute Rudjer Boskovic, Zagreb, Croatia}
{\tolerance=6000
P.~Bargassa\cmsorcid{0000-0001-8612-3332}, V.~Brigljevic\cmsorcid{0000-0001-5847-0062}, B.K.~Chitroda\cmsorcid{0000-0002-0220-8441}, D.~Ferencek\cmsorcid{0000-0001-9116-1202}, S.~Mishra\cmsorcid{0000-0002-3510-4833}, A.~Starodumov\cmsAuthorMark{16}\cmsorcid{0000-0001-9570-9255}, T.~Susa\cmsorcid{0000-0001-7430-2552}
\par}
\cmsinstitute{University of Cyprus, Nicosia, Cyprus}
{\tolerance=6000
A.~Attikis\cmsorcid{0000-0002-4443-3794}, K.~Christoforou\cmsorcid{0000-0003-2205-1100}, S.~Konstantinou\cmsorcid{0000-0003-0408-7636}, J.~Mousa\cmsorcid{0000-0002-2978-2718}, C.~Nicolaou, F.~Ptochos\cmsorcid{0000-0002-3432-3452}, P.A.~Razis\cmsorcid{0000-0002-4855-0162}, H.~Rykaczewski, H.~Saka\cmsorcid{0000-0001-7616-2573}, A.~Stepennov\cmsorcid{0000-0001-7747-6582}
\par}
\cmsinstitute{Charles University, Prague, Czech Republic}
{\tolerance=6000
M.~Finger\cmsorcid{0000-0002-7828-9970}, M.~Finger~Jr.\cmsorcid{0000-0003-3155-2484}, A.~Kveton\cmsorcid{0000-0001-8197-1914}
\par}
\cmsinstitute{Escuela Politecnica Nacional, Quito, Ecuador}
{\tolerance=6000
E.~Ayala\cmsorcid{0000-0002-0363-9198}
\par}
\cmsinstitute{Universidad San Francisco de Quito, Quito, Ecuador}
{\tolerance=6000
E.~Carrera~Jarrin\cmsorcid{0000-0002-0857-8507}
\par}
\cmsinstitute{Academy of Scientific Research and Technology of the Arab Republic of Egypt, Egyptian Network of High Energy Physics, Cairo, Egypt}
{\tolerance=6000
Y.~Assran\cmsAuthorMark{17}$^{, }$\cmsAuthorMark{18}, S.~Elgammal\cmsAuthorMark{18}
\par}
\cmsinstitute{Center for High Energy Physics (CHEP-FU), Fayoum University, El-Fayoum, Egypt}
{\tolerance=6000
M.~Abdullah~Al-Mashad\cmsorcid{0000-0002-7322-3374}, M.A.~Mahmoud\cmsorcid{0000-0001-8692-5458}
\par}
\cmsinstitute{National Institute of Chemical Physics and Biophysics, Tallinn, Estonia}
{\tolerance=6000
R.K.~Dewanjee\cmsAuthorMark{19}\cmsorcid{0000-0001-6645-6244}, K.~Ehataht\cmsorcid{0000-0002-2387-4777}, M.~Kadastik, T.~Lange\cmsorcid{0000-0001-6242-7331}, S.~Nandan\cmsorcid{0000-0002-9380-8919}, C.~Nielsen\cmsorcid{0000-0002-3532-8132}, J.~Pata\cmsorcid{0000-0002-5191-5759}, M.~Raidal\cmsorcid{0000-0001-7040-9491}, L.~Tani\cmsorcid{0000-0002-6552-7255}, C.~Veelken\cmsorcid{0000-0002-3364-916X}
\par}
\cmsinstitute{Department of Physics, University of Helsinki, Helsinki, Finland}
{\tolerance=6000
H.~Kirschenmann\cmsorcid{0000-0001-7369-2536}, K.~Osterberg\cmsorcid{0000-0003-4807-0414}, M.~Voutilainen\cmsorcid{0000-0002-5200-6477}
\par}
\cmsinstitute{Helsinki Institute of Physics, Helsinki, Finland}
{\tolerance=6000
S.~Bharthuar\cmsorcid{0000-0001-5871-9622}, E.~Br\"{u}cken\cmsorcid{0000-0001-6066-8756}, F.~Garcia\cmsorcid{0000-0002-4023-7964}, J.~Havukainen\cmsorcid{0000-0003-2898-6900}, K.T.S.~Kallonen\cmsorcid{0000-0001-9769-7163}, R.~Kinnunen, T.~Lamp\'{e}n\cmsorcid{0000-0002-8398-4249}, K.~Lassila-Perini\cmsorcid{0000-0002-5502-1795}, S.~Lehti\cmsorcid{0000-0003-1370-5598}, T.~Lind\'{e}n\cmsorcid{0009-0002-4847-8882}, M.~Lotti, L.~Martikainen\cmsorcid{0000-0003-1609-3515}, M.~Myllym\"{a}ki\cmsorcid{0000-0003-0510-3810}, M.m.~Rantanen\cmsorcid{0000-0002-6764-0016}, H.~Siikonen\cmsorcid{0000-0003-2039-5874}, E.~Tuominen\cmsorcid{0000-0002-7073-7767}, J.~Tuominiemi\cmsorcid{0000-0003-0386-8633}
\par}
\cmsinstitute{Lappeenranta-Lahti University of Technology, Lappeenranta, Finland}
{\tolerance=6000
P.~Luukka\cmsorcid{0000-0003-2340-4641}, H.~Petrow\cmsorcid{0000-0002-1133-5485}, T.~Tuuva$^{\textrm{\dag}}$
\par}
\cmsinstitute{IRFU, CEA, Universit\'{e} Paris-Saclay, Gif-sur-Yvette, France}
{\tolerance=6000
M.~Besancon\cmsorcid{0000-0003-3278-3671}, F.~Couderc\cmsorcid{0000-0003-2040-4099}, M.~Dejardin\cmsorcid{0009-0008-2784-615X}, D.~Denegri, J.L.~Faure, F.~Ferri\cmsorcid{0000-0002-9860-101X}, S.~Ganjour\cmsorcid{0000-0003-3090-9744}, P.~Gras\cmsorcid{0000-0002-3932-5967}, G.~Hamel~de~Monchenault\cmsorcid{0000-0002-3872-3592}, V.~Lohezic\cmsorcid{0009-0008-7976-851X}, J.~Malcles\cmsorcid{0000-0002-5388-5565}, J.~Rander, A.~Rosowsky\cmsorcid{0000-0001-7803-6650}, M.\"{O}.~Sahin\cmsorcid{0000-0001-6402-4050}, A.~Savoy-Navarro\cmsAuthorMark{20}\cmsorcid{0000-0002-9481-5168}, P.~Simkina\cmsorcid{0000-0002-9813-372X}, M.~Titov\cmsorcid{0000-0002-1119-6614}, M.~Tornago\cmsorcid{0000-0001-6768-1056}
\par}
\cmsinstitute{Laboratoire Leprince-Ringuet, CNRS/IN2P3, Ecole Polytechnique, Institut Polytechnique de Paris, Palaiseau, France}
{\tolerance=6000
C.~Baldenegro~Barrera\cmsorcid{0000-0002-6033-8885}, F.~Beaudette\cmsorcid{0000-0002-1194-8556}, A.~Buchot~Perraguin\cmsorcid{0000-0002-8597-647X}, P.~Busson\cmsorcid{0000-0001-6027-4511}, A.~Cappati\cmsorcid{0000-0003-4386-0564}, C.~Charlot\cmsorcid{0000-0002-4087-8155}, F.~Damas\cmsorcid{0000-0001-6793-4359}, O.~Davignon\cmsorcid{0000-0001-8710-992X}, A.~De~Wit\cmsorcid{0000-0002-5291-1661}, G.~Falmagne\cmsorcid{0000-0002-6762-3937}, B.A.~Fontana~Santos~Alves\cmsorcid{0000-0001-9752-0624}, S.~Ghosh\cmsorcid{0009-0006-5692-5688}, A.~Gilbert\cmsorcid{0000-0001-7560-5790}, R.~Granier~de~Cassagnac\cmsorcid{0000-0002-1275-7292}, A.~Hakimi\cmsorcid{0009-0008-2093-8131}, B.~Harikrishnan\cmsorcid{0000-0003-0174-4020}, L.~Kalipoliti\cmsorcid{0000-0002-5705-5059}, G.~Liu\cmsorcid{0000-0001-7002-0937}, J.~Motta\cmsorcid{0000-0003-0985-913X}, M.~Nguyen\cmsorcid{0000-0001-7305-7102}, C.~Ochando\cmsorcid{0000-0002-3836-1173}, L.~Portales\cmsorcid{0000-0002-9860-9185}, R.~Salerno\cmsorcid{0000-0003-3735-2707}, U.~Sarkar\cmsorcid{0000-0002-9892-4601}, J.B.~Sauvan\cmsorcid{0000-0001-5187-3571}, Y.~Sirois\cmsorcid{0000-0001-5381-4807}, A.~Tarabini\cmsorcid{0000-0001-7098-5317}, E.~Vernazza\cmsorcid{0000-0003-4957-2782}, A.~Zabi\cmsorcid{0000-0002-7214-0673}, A.~Zghiche\cmsorcid{0000-0002-1178-1450}
\par}
\cmsinstitute{Universit\'{e} de Strasbourg, CNRS, IPHC UMR 7178, Strasbourg, France}
{\tolerance=6000
J.-L.~Agram\cmsAuthorMark{21}\cmsorcid{0000-0001-7476-0158}, J.~Andrea\cmsorcid{0000-0002-8298-7560}, D.~Apparu\cmsorcid{0009-0004-1837-0496}, D.~Bloch\cmsorcid{0000-0002-4535-5273}, J.-M.~Brom\cmsorcid{0000-0003-0249-3622}, E.C.~Chabert\cmsorcid{0000-0003-2797-7690}, C.~Collard\cmsorcid{0000-0002-5230-8387}, S.~Falke\cmsorcid{0000-0002-0264-1632}, U.~Goerlach\cmsorcid{0000-0001-8955-1666}, C.~Grimault, R.~Haeberle\cmsorcid{0009-0007-5007-6723}, A.-C.~Le~Bihan\cmsorcid{0000-0002-8545-0187}, G.~Saha\cmsorcid{0000-0002-6125-1941}, M.A.~Sessini\cmsorcid{0000-0003-2097-7065}, P.~Van~Hove\cmsorcid{0000-0002-2431-3381}
\par}
\cmsinstitute{Institut de Physique des 2 Infinis de Lyon (IP2I ), Villeurbanne, France}
{\tolerance=6000
S.~Beauceron\cmsorcid{0000-0002-8036-9267}, B.~Blancon\cmsorcid{0000-0001-9022-1509}, G.~Boudoul\cmsorcid{0009-0002-9897-8439}, N.~Chanon\cmsorcid{0000-0002-2939-5646}, J.~Choi\cmsorcid{0000-0002-6024-0992}, D.~Contardo\cmsorcid{0000-0001-6768-7466}, P.~Depasse\cmsorcid{0000-0001-7556-2743}, C.~Dozen\cmsAuthorMark{22}\cmsorcid{0000-0002-4301-634X}, H.~El~Mamouni, J.~Fay\cmsorcid{0000-0001-5790-1780}, S.~Gascon\cmsorcid{0000-0002-7204-1624}, M.~Gouzevitch\cmsorcid{0000-0002-5524-880X}, C.~Greenberg, G.~Grenier\cmsorcid{0000-0002-1976-5877}, B.~Ille\cmsorcid{0000-0002-8679-3878}, I.B.~Laktineh, M.~Lethuillier\cmsorcid{0000-0001-6185-2045}, L.~Mirabito, S.~Perries, A.~Purohit\cmsorcid{0000-0003-0881-612X}, M.~Vander~Donckt\cmsorcid{0000-0002-9253-8611}, P.~Verdier\cmsorcid{0000-0003-3090-2948}, J.~Xiao\cmsorcid{0000-0002-7860-3958}
\par}
\cmsinstitute{Georgian Technical University, Tbilisi, Georgia}
{\tolerance=6000
I.~Lomidze\cmsorcid{0009-0002-3901-2765}, T.~Toriashvili\cmsAuthorMark{23}\cmsorcid{0000-0003-1655-6874}, Z.~Tsamalaidze\cmsAuthorMark{16}\cmsorcid{0000-0001-5377-3558}
\par}
\cmsinstitute{RWTH Aachen University, I. Physikalisches Institut, Aachen, Germany}
{\tolerance=6000
V.~Botta\cmsorcid{0000-0003-1661-9513}, L.~Feld\cmsorcid{0000-0001-9813-8646}, K.~Klein\cmsorcid{0000-0002-1546-7880}, M.~Lipinski\cmsorcid{0000-0002-6839-0063}, D.~Meuser\cmsorcid{0000-0002-2722-7526}, A.~Pauls\cmsorcid{0000-0002-8117-5376}, N.~R\"{o}wert\cmsorcid{0000-0002-4745-5470}, M.~Teroerde\cmsorcid{0000-0002-5892-1377}
\par}
\cmsinstitute{RWTH Aachen University, III. Physikalisches Institut A, Aachen, Germany}
{\tolerance=6000
S.~Diekmann\cmsorcid{0009-0004-8867-0881}, A.~Dodonova\cmsorcid{0000-0002-5115-8487}, N.~Eich\cmsorcid{0000-0001-9494-4317}, D.~Eliseev\cmsorcid{0000-0001-5844-8156}, F.~Engelke\cmsorcid{0000-0002-9288-8144}, M.~Erdmann\cmsorcid{0000-0002-1653-1303}, P.~Fackeldey\cmsorcid{0000-0003-4932-7162}, B.~Fischer\cmsorcid{0000-0002-3900-3482}, T.~Hebbeker\cmsorcid{0000-0002-9736-266X}, K.~Hoepfner\cmsorcid{0000-0002-2008-8148}, F.~Ivone\cmsorcid{0000-0002-2388-5548}, A.~Jung\cmsorcid{0000-0002-2511-1490}, M.y.~Lee\cmsorcid{0000-0002-4430-1695}, L.~Mastrolorenzo, M.~Merschmeyer\cmsorcid{0000-0003-2081-7141}, A.~Meyer\cmsorcid{0000-0001-9598-6623}, S.~Mukherjee\cmsorcid{0000-0001-6341-9982}, D.~Noll\cmsorcid{0000-0002-0176-2360}, A.~Novak\cmsorcid{0000-0002-0389-5896}, F.~Nowotny, A.~Pozdnyakov\cmsorcid{0000-0003-3478-9081}, Y.~Rath, W.~Redjeb\cmsorcid{0000-0001-9794-8292}, F.~Rehm, H.~Reithler\cmsorcid{0000-0003-4409-702X}, V.~Sarkisovi\cmsorcid{0000-0001-9430-5419}, A.~Schmidt\cmsorcid{0000-0003-2711-8984}, A.~Sharma\cmsorcid{0000-0002-5295-1460}, J.L.~Spah\cmsorcid{0000-0002-5215-3258}, A.~Stein\cmsorcid{0000-0003-0713-811X}, F.~Torres~Da~Silva~De~Araujo\cmsAuthorMark{24}\cmsorcid{0000-0002-4785-3057}, L.~Vigilante, S.~Wiedenbeck\cmsorcid{0000-0002-4692-9304}, S.~Zaleski
\par}
\cmsinstitute{RWTH Aachen University, III. Physikalisches Institut B, Aachen, Germany}
{\tolerance=6000
C.~Dziwok\cmsorcid{0000-0001-9806-0244}, G.~Fl\"{u}gge\cmsorcid{0000-0003-3681-9272}, W.~Haj~Ahmad\cmsAuthorMark{25}\cmsorcid{0000-0003-1491-0446}, T.~Kress\cmsorcid{0000-0002-2702-8201}, A.~Nowack\cmsorcid{0000-0002-3522-5926}, O.~Pooth\cmsorcid{0000-0001-6445-6160}, A.~Stahl\cmsorcid{0000-0002-8369-7506}, T.~Ziemons\cmsorcid{0000-0003-1697-2130}, A.~Zotz\cmsorcid{0000-0002-1320-1712}
\par}
\cmsinstitute{Deutsches Elektronen-Synchrotron, Hamburg, Germany}
{\tolerance=6000
H.~Aarup~Petersen\cmsorcid{0009-0005-6482-7466}, M.~Aldaya~Martin\cmsorcid{0000-0003-1533-0945}, J.~Alimena\cmsorcid{0000-0001-6030-3191}, S.~Amoroso, Y.~An\cmsorcid{0000-0003-1299-1879}, S.~Baxter\cmsorcid{0009-0008-4191-6716}, M.~Bayatmakou\cmsorcid{0009-0002-9905-0667}, H.~Becerril~Gonzalez\cmsorcid{0000-0001-5387-712X}, O.~Behnke\cmsorcid{0000-0002-4238-0991}, A.~Belvedere\cmsorcid{0000-0002-2802-8203}, S.~Bhattacharya\cmsorcid{0000-0002-3197-0048}, F.~Blekman\cmsAuthorMark{26}\cmsorcid{0000-0002-7366-7098}, K.~Borras\cmsAuthorMark{27}\cmsorcid{0000-0003-1111-249X}, D.~Brunner\cmsorcid{0000-0001-9518-0435}, A.~Campbell\cmsorcid{0000-0003-4439-5748}, A.~Cardini\cmsorcid{0000-0003-1803-0999}, C.~Cheng, F.~Colombina\cmsorcid{0009-0008-7130-100X}, S.~Consuegra~Rodr\'{i}guez\cmsorcid{0000-0002-1383-1837}, G.~Correia~Silva\cmsorcid{0000-0001-6232-3591}, M.~De~Silva\cmsorcid{0000-0002-5804-6226}, G.~Eckerlin, D.~Eckstein\cmsorcid{0000-0002-7366-6562}, L.I.~Estevez~Banos\cmsorcid{0000-0001-6195-3102}, O.~Filatov\cmsorcid{0000-0001-9850-6170}, E.~Gallo\cmsAuthorMark{26}\cmsorcid{0000-0001-7200-5175}, A.~Geiser\cmsorcid{0000-0003-0355-102X}, A.~Giraldi\cmsorcid{0000-0003-4423-2631}, G.~Greau, V.~Guglielmi\cmsorcid{0000-0003-3240-7393}, M.~Guthoff\cmsorcid{0000-0002-3974-589X}, A.~Hinzmann\cmsorcid{0000-0002-2633-4696}, A.~Jafari\cmsAuthorMark{28}\cmsorcid{0000-0001-7327-1870}, L.~Jeppe\cmsorcid{0000-0002-1029-0318}, N.Z.~Jomhari\cmsorcid{0000-0001-9127-7408}, B.~Kaech\cmsorcid{0000-0002-1194-2306}, M.~Kasemann\cmsorcid{0000-0002-0429-2448}, H.~Kaveh\cmsorcid{0000-0002-3273-5859}, C.~Kleinwort\cmsorcid{0000-0002-9017-9504}, R.~Kogler\cmsorcid{0000-0002-5336-4399}, M.~Komm\cmsorcid{0000-0002-7669-4294}, D.~Kr\"{u}cker\cmsorcid{0000-0003-1610-8844}, W.~Lange, D.~Leyva~Pernia\cmsorcid{0009-0009-8755-3698}, K.~Lipka\cmsAuthorMark{29}\cmsorcid{0000-0002-8427-3748}, W.~Lohmann\cmsAuthorMark{30}\cmsorcid{0000-0002-8705-0857}, R.~Mankel\cmsorcid{0000-0003-2375-1563}, I.-A.~Melzer-Pellmann\cmsorcid{0000-0001-7707-919X}, M.~Mendizabal~Morentin\cmsorcid{0000-0002-6506-5177}, J.~Metwally, A.B.~Meyer\cmsorcid{0000-0001-8532-2356}, G.~Milella\cmsorcid{0000-0002-2047-951X}, A.~Mussgiller\cmsorcid{0000-0002-8331-8166}, L.P.~NAIR\cmsorcid{0000-0002-2351-9265}, A.~N\"{u}rnberg\cmsorcid{0000-0002-7876-3134}, Y.~Otarid, J.~Park\cmsorcid{0000-0002-4683-6669}, D.~P\'{e}rez~Ad\'{a}n\cmsorcid{0000-0003-3416-0726}, E.~Ranken\cmsorcid{0000-0001-7472-5029}, A.~Raspereza\cmsorcid{0000-0003-2167-498X}, B.~Ribeiro~Lopes\cmsorcid{0000-0003-0823-447X}, J.~R\"{u}benach, A.~Saggio\cmsorcid{0000-0002-7385-3317}, M.~Scham\cmsAuthorMark{31}$^{, }$\cmsAuthorMark{27}\cmsorcid{0000-0001-9494-2151}, S.~Schnake\cmsAuthorMark{27}\cmsorcid{0000-0003-3409-6584}, P.~Sch\"{u}tze\cmsorcid{0000-0003-4802-6990}, C.~Schwanenberger\cmsAuthorMark{26}\cmsorcid{0000-0001-6699-6662}, D.~Selivanova\cmsorcid{0000-0002-7031-9434}, M.~Shchedrolosiev\cmsorcid{0000-0003-3510-2093}, R.E.~Sosa~Ricardo\cmsorcid{0000-0002-2240-6699}, D.~Stafford, F.~Vazzoler\cmsorcid{0000-0001-8111-9318}, A.~Ventura~Barroso\cmsorcid{0000-0003-3233-6636}, R.~Walsh\cmsorcid{0000-0002-3872-4114}, Q.~Wang\cmsorcid{0000-0003-1014-8677}, Y.~Wen\cmsorcid{0000-0002-8724-9604}, K.~Wichmann, L.~Wiens\cmsAuthorMark{27}\cmsorcid{0000-0002-4423-4461}, C.~Wissing\cmsorcid{0000-0002-5090-8004}, Y.~Yang\cmsorcid{0009-0009-3430-0558}, A.~Zimermmane~Castro~Santos\cmsorcid{0000-0001-9302-3102}
\par}
\cmsinstitute{University of Hamburg, Hamburg, Germany}
{\tolerance=6000
A.~Albrecht\cmsorcid{0000-0001-6004-6180}, S.~Albrecht\cmsorcid{0000-0002-5960-6803}, M.~Antonello\cmsorcid{0000-0001-9094-482X}, S.~Bein\cmsorcid{0000-0001-9387-7407}, L.~Benato\cmsorcid{0000-0001-5135-7489}, M.~Bonanomi\cmsorcid{0000-0003-3629-6264}, P.~Connor\cmsorcid{0000-0003-2500-1061}, M.~Eich, K.~El~Morabit\cmsorcid{0000-0001-5886-220X}, Y.~Fischer\cmsorcid{0000-0002-3184-1457}, A.~Fr\"{o}hlich, C.~Garbers\cmsorcid{0000-0001-5094-2256}, E.~Garutti\cmsorcid{0000-0003-0634-5539}, A.~Grohsjean\cmsorcid{0000-0003-0748-8494}, M.~Hajheidari, J.~Haller\cmsorcid{0000-0001-9347-7657}, H.R.~Jabusch\cmsorcid{0000-0003-2444-1014}, G.~Kasieczka\cmsorcid{0000-0003-3457-2755}, P.~Keicher, R.~Klanner\cmsorcid{0000-0002-7004-9227}, W.~Korcari\cmsorcid{0000-0001-8017-5502}, T.~Kramer\cmsorcid{0000-0002-7004-0214}, V.~Kutzner\cmsorcid{0000-0003-1985-3807}, F.~Labe\cmsorcid{0000-0002-1870-9443}, J.~Lange\cmsorcid{0000-0001-7513-6330}, A.~Lobanov\cmsorcid{0000-0002-5376-0877}, C.~Matthies\cmsorcid{0000-0001-7379-4540}, A.~Mehta\cmsorcid{0000-0002-0433-4484}, L.~Moureaux\cmsorcid{0000-0002-2310-9266}, M.~Mrowietz, A.~Nigamova\cmsorcid{0000-0002-8522-8500}, Y.~Nissan, A.~Paasch\cmsorcid{0000-0002-2208-5178}, K.J.~Pena~Rodriguez\cmsorcid{0000-0002-2877-9744}, T.~Quadfasel\cmsorcid{0000-0003-2360-351X}, B.~Raciti\cmsorcid{0009-0005-5995-6685}, M.~Rieger\cmsorcid{0000-0003-0797-2606}, D.~Savoiu\cmsorcid{0000-0001-6794-7475}, J.~Schindler\cmsorcid{0009-0006-6551-0660}, P.~Schleper\cmsorcid{0000-0001-5628-6827}, M.~Schr\"{o}der\cmsorcid{0000-0001-8058-9828}, J.~Schwandt\cmsorcid{0000-0002-0052-597X}, M.~Sommerhalder\cmsorcid{0000-0001-5746-7371}, H.~Stadie\cmsorcid{0000-0002-0513-8119}, G.~Steinbr\"{u}ck\cmsorcid{0000-0002-8355-2761}, A.~Tews, M.~Wolf\cmsorcid{0000-0003-3002-2430}
\par}
\cmsinstitute{Karlsruher Institut fuer Technologie, Karlsruhe, Germany}
{\tolerance=6000
S.~Brommer\cmsorcid{0000-0001-8988-2035}, M.~Burkart, E.~Butz\cmsorcid{0000-0002-2403-5801}, T.~Chwalek\cmsorcid{0000-0002-8009-3723}, A.~Dierlamm\cmsorcid{0000-0001-7804-9902}, A.~Droll, N.~Faltermann\cmsorcid{0000-0001-6506-3107}, M.~Giffels\cmsorcid{0000-0003-0193-3032}, A.~Gottmann\cmsorcid{0000-0001-6696-349X}, F.~Hartmann\cmsAuthorMark{32}\cmsorcid{0000-0001-8989-8387}, R.~Hofsaess\cmsorcid{0009-0008-4575-5729}, M.~Horzela\cmsorcid{0000-0002-3190-7962}, U.~Husemann\cmsorcid{0000-0002-6198-8388}, J.~Kieseler\cmsorcid{0000-0003-1644-7678}, M.~Klute\cmsorcid{0000-0002-0869-5631}, R.~Koppenh\"{o}fer\cmsorcid{0000-0002-6256-5715}, J.M.~Lawhorn\cmsorcid{0000-0002-8597-9259}, M.~Link, A.~Lintuluoto\cmsorcid{0000-0002-0726-1452}, S.~Maier\cmsorcid{0000-0001-9828-9778}, S.~Mitra\cmsorcid{0000-0002-3060-2278}, M.~Mormile\cmsorcid{0000-0003-0456-7250}, Th.~M\"{u}ller\cmsorcid{0000-0003-4337-0098}, M.~Neukum, M.~Oh\cmsorcid{0000-0003-2618-9203}, M.~Presilla\cmsorcid{0000-0003-2808-7315}, G.~Quast\cmsorcid{0000-0002-4021-4260}, K.~Rabbertz\cmsorcid{0000-0001-7040-9846}, B.~Regnery\cmsorcid{0000-0003-1539-923X}, N.~Shadskiy\cmsorcid{0000-0001-9894-2095}, I.~Shvetsov\cmsorcid{0000-0002-7069-9019}, H.J.~Simonis\cmsorcid{0000-0002-7467-2980}, N.~Trevisani\cmsorcid{0000-0002-5223-9342}, R.~Ulrich\cmsorcid{0000-0002-2535-402X}, J.~van~der~Linden\cmsorcid{0000-0002-7174-781X}, R.F.~Von~Cube\cmsorcid{0000-0002-6237-5209}, M.~Wassmer\cmsorcid{0000-0002-0408-2811}, S.~Wieland\cmsorcid{0000-0003-3887-5358}, F.~Wittig, R.~Wolf\cmsorcid{0000-0001-9456-383X}, S.~Wunsch, X.~Zuo\cmsorcid{0000-0002-0029-493X}
\par}
\cmsinstitute{Institute of Nuclear and Particle Physics (INPP), NCSR Demokritos, Aghia Paraskevi, Greece}
{\tolerance=6000
G.~Anagnostou, P.~Assiouras\cmsorcid{0000-0002-5152-9006}, G.~Daskalakis\cmsorcid{0000-0001-6070-7698}, A.~Kyriakis, A.~Papadopoulos\cmsAuthorMark{32}, A.~Stakia\cmsorcid{0000-0001-6277-7171}
\par}
\cmsinstitute{National and Kapodistrian University of Athens, Athens, Greece}
{\tolerance=6000
P.~Kontaxakis\cmsorcid{0000-0002-4860-5979}, G.~Melachroinos, A.~Panagiotou, I.~Papavergou\cmsorcid{0000-0002-7992-2686}, I.~Paraskevas\cmsorcid{0000-0002-2375-5401}, N.~Saoulidou\cmsorcid{0000-0001-6958-4196}, K.~Theofilatos\cmsorcid{0000-0001-8448-883X}, E.~Tziaferi\cmsorcid{0000-0003-4958-0408}, K.~Vellidis\cmsorcid{0000-0001-5680-8357}, I.~Zisopoulos\cmsorcid{0000-0001-5212-4353}
\par}
\cmsinstitute{National Technical University of Athens, Athens, Greece}
{\tolerance=6000
G.~Bakas\cmsorcid{0000-0003-0287-1937}, T.~Chatzistavrou, G.~Karapostoli\cmsorcid{0000-0002-4280-2541}, K.~Kousouris\cmsorcid{0000-0002-6360-0869}, I.~Papakrivopoulos\cmsorcid{0000-0002-8440-0487}, E.~Siamarkou, G.~Tsipolitis, A.~Zacharopoulou
\par}
\cmsinstitute{University of Io\'{a}nnina, Io\'{a}nnina, Greece}
{\tolerance=6000
K.~Adamidis, I.~Bestintzanos, I.~Evangelou\cmsorcid{0000-0002-5903-5481}, C.~Foudas, P.~Gianneios\cmsorcid{0009-0003-7233-0738}, C.~Kamtsikis, P.~Katsoulis, P.~Kokkas\cmsorcid{0009-0009-3752-6253}, P.G.~Kosmoglou~Kioseoglou\cmsorcid{0000-0002-7440-4396}, N.~Manthos\cmsorcid{0000-0003-3247-8909}, I.~Papadopoulos\cmsorcid{0000-0002-9937-3063}, J.~Strologas\cmsorcid{0000-0002-2225-7160}
\par}
\cmsinstitute{MTA-ELTE Lend\"{u}let CMS Particle and Nuclear Physics Group, E\"{o}tv\"{o}s Lor\'{a}nd University, Budapest, Hungary}
{\tolerance=6000
M.~Csan\'{a}d\cmsorcid{0000-0002-3154-6925}, K.~Farkas\cmsorcid{0000-0003-1740-6974}, M.M.A.~Gadallah\cmsAuthorMark{33}\cmsorcid{0000-0002-8305-6661}, \'{A}.~Kadlecsik\cmsorcid{0000-0001-5559-0106}, P.~Major\cmsorcid{0000-0002-5476-0414}, K.~Mandal\cmsorcid{0000-0002-3966-7182}, G.~P\'{a}sztor\cmsorcid{0000-0003-0707-9762}, A.J.~R\'{a}dl\cmsAuthorMark{34}\cmsorcid{0000-0001-8810-0388}, G.I.~Veres\cmsorcid{0000-0002-5440-4356}
\par}
\cmsinstitute{Wigner Research Centre for Physics, Budapest, Hungary}
{\tolerance=6000
M.~Bart\'{o}k\cmsAuthorMark{35}\cmsorcid{0000-0002-4440-2701}, C.~Hajdu\cmsorcid{0000-0002-7193-800X}, D.~Horvath\cmsAuthorMark{36}$^{, }$\cmsAuthorMark{37}\cmsorcid{0000-0003-0091-477X}, F.~Sikler\cmsorcid{0000-0001-9608-3901}, V.~Veszpremi\cmsorcid{0000-0001-9783-0315}
\par}
\cmsinstitute{Faculty of Informatics, University of Debrecen, Debrecen, Hungary}
{\tolerance=6000
P.~Raics, B.~Ujvari\cmsAuthorMark{38}\cmsorcid{0000-0003-0498-4265}, G.~Zilizi\cmsorcid{0000-0002-0480-0000}
\par}
\cmsinstitute{Institute of Nuclear Research ATOMKI, Debrecen, Hungary}
{\tolerance=6000
G.~Bencze, S.~Czellar, J.~Karancsi\cmsAuthorMark{35}\cmsorcid{0000-0003-0802-7665}, J.~Molnar, Z.~Szillasi
\par}
\cmsinstitute{Karoly Robert Campus, MATE Institute of Technology, Gyongyos, Hungary}
{\tolerance=6000
T.~Csorgo\cmsAuthorMark{34}\cmsorcid{0000-0002-9110-9663}, F.~Nemes\cmsAuthorMark{34}\cmsorcid{0000-0002-1451-6484}, T.~Novak\cmsorcid{0000-0001-6253-4356}
\par}
\cmsinstitute{Panjab University, Chandigarh, India}
{\tolerance=6000
J.~Babbar\cmsorcid{0000-0002-4080-4156}, S.~Bansal\cmsorcid{0000-0003-1992-0336}, S.B.~Beri, V.~Bhatnagar\cmsorcid{0000-0002-8392-9610}, G.~Chaudhary\cmsorcid{0000-0003-0168-3336}, S.~Chauhan\cmsorcid{0000-0001-6974-4129}, N.~Dhingra\cmsAuthorMark{39}\cmsorcid{0000-0002-7200-6204}, A.~Kaur\cmsorcid{0000-0002-1640-9180}, A.~Kaur\cmsorcid{0000-0003-3609-4777}, H.~Kaur\cmsorcid{0000-0002-8659-7092}, M.~Kaur\cmsorcid{0000-0002-3440-2767}, S.~Kumar\cmsorcid{0000-0001-9212-9108}, M.~Meena\cmsorcid{0000-0003-4536-3967}, K.~Sandeep\cmsorcid{0000-0002-3220-3668}, T.~Sheokand, J.B.~Singh\cmsorcid{0000-0001-9029-2462}, A.~Singla\cmsorcid{0000-0003-2550-139X}
\par}
\cmsinstitute{University of Delhi, Delhi, India}
{\tolerance=6000
A.~Ahmed\cmsorcid{0000-0002-4500-8853}, A.~Bhardwaj\cmsorcid{0000-0002-7544-3258}, A.~Chhetri\cmsorcid{0000-0001-7495-1923}, B.C.~Choudhary\cmsorcid{0000-0001-5029-1887}, A.~Kumar\cmsorcid{0000-0003-3407-4094}, M.~Naimuddin\cmsorcid{0000-0003-4542-386X}, K.~Ranjan\cmsorcid{0000-0002-5540-3750}, S.~Saumya\cmsorcid{0000-0001-7842-9518}
\par}
\cmsinstitute{Saha Institute of Nuclear Physics, HBNI, Kolkata, India}
{\tolerance=6000
S.~Acharya\cmsAuthorMark{40}, S.~Baradia\cmsorcid{0000-0001-9860-7262}, S.~Barman\cmsAuthorMark{41}\cmsorcid{0000-0001-8891-1674}, S.~Bhattacharya\cmsorcid{0000-0002-8110-4957}, D.~Bhowmik, S.~Dutta\cmsorcid{0000-0001-9650-8121}, S.~Dutta, P.~Palit\cmsorcid{0000-0002-1948-029X}, B.~Sahu\cmsAuthorMark{40}\cmsorcid{0000-0002-8073-5140}, S.~Sarkar
\par}
\cmsinstitute{Indian Institute of Technology Madras, Madras, India}
{\tolerance=6000
M.M.~Ameen\cmsorcid{0000-0002-1909-9843}, P.K.~Behera\cmsorcid{0000-0002-1527-2266}, S.C.~Behera\cmsorcid{0000-0002-0798-2727}, S.~Chatterjee\cmsorcid{0000-0003-0185-9872}, P.~Jana\cmsorcid{0000-0001-5310-5170}, P.~Kalbhor\cmsorcid{0000-0002-5892-3743}, J.R.~Komaragiri\cmsAuthorMark{42}\cmsorcid{0000-0002-9344-6655}, D.~Kumar\cmsAuthorMark{42}\cmsorcid{0000-0002-6636-5331}, L.~Panwar\cmsAuthorMark{42}\cmsorcid{0000-0003-2461-4907}, R.~Pradhan\cmsorcid{0000-0001-7000-6510}, P.R.~Pujahari\cmsorcid{0000-0002-0994-7212}, N.R.~Saha\cmsorcid{0000-0002-7954-7898}, A.~Sharma\cmsorcid{0000-0002-0688-923X}, A.K.~Sikdar\cmsorcid{0000-0002-5437-5217}, S.~Verma\cmsorcid{0000-0003-1163-6955}
\par}
\cmsinstitute{Tata Institute of Fundamental Research-A, Mumbai, India}
{\tolerance=6000
T.~Aziz, I.~Das\cmsorcid{0000-0002-5437-2067}, S.~Dugad, M.~Kumar\cmsorcid{0000-0003-0312-057X}, G.B.~Mohanty\cmsorcid{0000-0001-6850-7666}, P.~Suryadevara
\par}
\cmsinstitute{Tata Institute of Fundamental Research-B, Mumbai, India}
{\tolerance=6000
A.~Bala\cmsorcid{0000-0003-2565-1718}, S.~Banerjee\cmsorcid{0000-0002-7953-4683}, R.M.~Chatterjee, M.~Guchait\cmsorcid{0009-0004-0928-7922}, Sh.~Jain\cmsorcid{0000-0003-1770-5309}, S.~Karmakar\cmsorcid{0000-0001-9715-5663}, S.~Kumar\cmsorcid{0000-0002-2405-915X}, G.~Majumder\cmsorcid{0000-0002-3815-5222}, K.~Mazumdar\cmsorcid{0000-0003-3136-1653}, S.~Mukherjee\cmsorcid{0000-0003-3122-0594}, S.~Parolia\cmsorcid{0000-0002-9566-2490}, A.~Thachayath\cmsorcid{0000-0001-6545-0350}
\par}
\cmsinstitute{National Institute of Science Education and Research, An OCC of Homi Bhabha National Institute, Bhubaneswar, Odisha, India}
{\tolerance=6000
S.~Bahinipati\cmsAuthorMark{43}\cmsorcid{0000-0002-3744-5332}, A.K.~Das, C.~Kar\cmsorcid{0000-0002-6407-6974}, D.~Maity\cmsAuthorMark{44}\cmsorcid{0000-0002-1989-6703}, P.~Mal\cmsorcid{0000-0002-0870-8420}, T.~Mishra\cmsorcid{0000-0002-2121-3932}, V.K.~Muraleedharan~Nair~Bindhu\cmsAuthorMark{44}\cmsorcid{0000-0003-4671-815X}, K.~Naskar\cmsAuthorMark{44}\cmsorcid{0000-0003-0638-4378}, A.~Nayak\cmsAuthorMark{44}\cmsorcid{0000-0002-7716-4981}, P.~Sadangi, P.~Saha\cmsorcid{0000-0002-7013-8094}, S.K.~Swain\cmsorcid{0000-0001-6871-3937}, S.~Varghese\cmsAuthorMark{44}\cmsorcid{0009-0000-1318-8266}, D.~Vats\cmsAuthorMark{44}\cmsorcid{0009-0007-8224-4664}
\par}
\cmsinstitute{Indian Institute of Science Education and Research (IISER), Pune, India}
{\tolerance=6000
A.~Alpana\cmsorcid{0000-0003-3294-2345}, S.~Dube\cmsorcid{0000-0002-5145-3777}, B.~Gomber\cmsAuthorMark{40}\cmsorcid{0000-0002-4446-0258}, B.~Kansal\cmsorcid{0000-0002-6604-1011}, A.~Laha\cmsorcid{0000-0001-9440-7028}, A.~Rastogi\cmsorcid{0000-0003-1245-6710}, S.~Sharma\cmsorcid{0000-0001-6886-0726}
\par}
\cmsinstitute{Isfahan University of Technology, Isfahan, Iran}
{\tolerance=6000
H.~Bakhshiansohi\cmsAuthorMark{45}\cmsorcid{0000-0001-5741-3357}, E.~Khazaie\cmsAuthorMark{46}\cmsorcid{0000-0001-9810-7743}, M.~Zeinali\cmsAuthorMark{47}\cmsorcid{0000-0001-8367-6257}
\par}
\cmsinstitute{Institute for Research in Fundamental Sciences (IPM), Tehran, Iran}
{\tolerance=6000
S.~Chenarani\cmsAuthorMark{48}\cmsorcid{0000-0002-1425-076X}, S.M.~Etesami\cmsorcid{0000-0001-6501-4137}, M.~Khakzad\cmsorcid{0000-0002-2212-5715}, M.~Mohammadi~Najafabadi\cmsorcid{0000-0001-6131-5987}
\par}
\cmsinstitute{University College Dublin, Dublin, Ireland}
{\tolerance=6000
M.~Grunewald\cmsorcid{0000-0002-5754-0388}
\par}
\cmsinstitute{INFN Sezione di Bari$^{a}$, Universit\`{a} di Bari$^{b}$, Politecnico di Bari$^{c}$, Bari, Italy}
{\tolerance=6000
M.~Abbrescia$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-8727-7544}, R.~Aly$^{a}$$^{, }$$^{c}$$^{, }$\cmsAuthorMark{49}\cmsorcid{0000-0001-6808-1335}, A.~Colaleo$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-0711-6319}, D.~Creanza$^{a}$$^{, }$$^{c}$\cmsorcid{0000-0001-6153-3044}, B.~D`~Anzi$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-9361-3142}, N.~De~Filippis$^{a}$$^{, }$$^{c}$\cmsorcid{0000-0002-0625-6811}, M.~De~Palma$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-8240-1913}, A.~Di~Florio$^{a}$$^{, }$$^{c}$\cmsorcid{0000-0003-3719-8041}, W.~Elmetenawee$^{a}$$^{, }$$^{b}$$^{, }$\cmsAuthorMark{49}\cmsorcid{0000-0001-7069-0252}, L.~Fiore$^{a}$\cmsorcid{0000-0002-9470-1320}, G.~Iaselli$^{a}$$^{, }$$^{c}$\cmsorcid{0000-0003-2546-5341}, M.~Louka$^{a}$$^{, }$$^{b}$, G.~Maggi$^{a}$$^{, }$$^{c}$\cmsorcid{0000-0001-5391-7689}, M.~Maggi$^{a}$\cmsorcid{0000-0002-8431-3922}, I.~Margjeka$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-3198-3025}, V.~Mastrapasqua$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-9082-5924}, S.~My$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-9938-2680}, S.~Nuzzo$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-1089-6317}, A.~Pellecchia$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-3279-6114}, A.~Pompili$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-1291-4005}, G.~Pugliese$^{a}$$^{, }$$^{c}$\cmsorcid{0000-0001-5460-2638}, R.~Radogna$^{a}$\cmsorcid{0000-0002-1094-5038}, G.~Ramirez-Sanchez$^{a}$$^{, }$$^{c}$\cmsorcid{0000-0001-7804-5514}, D.~Ramos$^{a}$\cmsorcid{0000-0002-7165-1017}, A.~Ranieri$^{a}$\cmsorcid{0000-0001-7912-4062}, L.~Silvestris$^{a}$\cmsorcid{0000-0002-8985-4891}, F.M.~Simone$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-1924-983X}, \"{U}.~S\"{o}zbilir$^{a}$\cmsorcid{0000-0001-6833-3758}, A.~Stamerra$^{a}$\cmsorcid{0000-0003-1434-1968}, R.~Venditti$^{a}$\cmsorcid{0000-0001-6925-8649}, P.~Verwilligen$^{a}$\cmsorcid{0000-0002-9285-8631}, A.~Zaza$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-0969-7284}
\par}
\cmsinstitute{INFN Sezione di Bologna$^{a}$, Universit\`{a} di Bologna$^{b}$, Bologna, Italy}
{\tolerance=6000
G.~Abbiendi$^{a}$\cmsorcid{0000-0003-4499-7562}, C.~Battilana$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-3753-3068}, D.~Bonacorsi$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-0835-9574}, L.~Borgonovi$^{a}$\cmsorcid{0000-0001-8679-4443}, P.~Capiluppi$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-4485-1897}, A.~Castro$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-2527-0456}, F.R.~Cavallo$^{a}$\cmsorcid{0000-0002-0326-7515}, M.~Cuffiani$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-2510-5039}, G.M.~Dallavalle$^{a}$\cmsorcid{0000-0002-8614-0420}, T.~Diotalevi$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-0780-8785}, F.~Fabbri$^{a}$\cmsorcid{0000-0002-8446-9660}, A.~Fanfani$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-2256-4117}, D.~Fasanella$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-2926-2691}, P.~Giacomelli$^{a}$\cmsorcid{0000-0002-6368-7220}, L.~Giommi$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-3539-4313}, C.~Grandi$^{a}$\cmsorcid{0000-0001-5998-3070}, L.~Guiducci$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-6013-8293}, S.~Lo~Meo$^{a}$$^{, }$\cmsAuthorMark{50}\cmsorcid{0000-0003-3249-9208}, L.~Lunerti$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-8932-0283}, S.~Marcellini$^{a}$\cmsorcid{0000-0002-1233-8100}, G.~Masetti$^{a}$\cmsorcid{0000-0002-6377-800X}, F.L.~Navarria$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-7961-4889}, A.~Perrotta$^{a}$\cmsorcid{0000-0002-7996-7139}, F.~Primavera$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-6253-8656}, A.M.~Rossi$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-5973-1305}, T.~Rovelli$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-9746-4842}, G.P.~Siroli$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-3528-4125}
\par}
\cmsinstitute{INFN Sezione di Catania$^{a}$, Universit\`{a} di Catania$^{b}$, Catania, Italy}
{\tolerance=6000
S.~Costa$^{a}$$^{, }$$^{b}$$^{, }$\cmsAuthorMark{51}\cmsorcid{0000-0001-9919-0569}, A.~Di~Mattia$^{a}$\cmsorcid{0000-0002-9964-015X}, R.~Potenza$^{a}$$^{, }$$^{b}$, A.~Tricomi$^{a}$$^{, }$$^{b}$$^{, }$\cmsAuthorMark{51}\cmsorcid{0000-0002-5071-5501}, C.~Tuve$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-0739-3153}
\par}
\cmsinstitute{INFN Sezione di Firenze$^{a}$, Universit\`{a} di Firenze$^{b}$, Firenze, Italy}
{\tolerance=6000
G.~Barbagli$^{a}$\cmsorcid{0000-0002-1738-8676}, G.~Bardelli$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-4662-3305}, B.~Camaiani$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-6396-622X}, A.~Cassese$^{a}$\cmsorcid{0000-0003-3010-4516}, R.~Ceccarelli$^{a}$\cmsorcid{0000-0003-3232-9380}, V.~Ciulli$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-1947-3396}, C.~Civinini$^{a}$\cmsorcid{0000-0002-4952-3799}, R.~D'Alessandro$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-7997-0306}, E.~Focardi$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-3763-5267}, T.~Kello$^{a}$, G.~Latino$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-4098-3502}, P.~Lenzi$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-6927-8807}, M.~Lizzo$^{a}$\cmsorcid{0000-0001-7297-2624}, M.~Meschini$^{a}$\cmsorcid{0000-0002-9161-3990}, S.~Paoletti$^{a}$\cmsorcid{0000-0003-3592-9509}, A.~Papanastassiou$^{a}$$^{, }$$^{b}$, G.~Sguazzoni$^{a}$\cmsorcid{0000-0002-0791-3350}, L.~Viliani$^{a}$\cmsorcid{0000-0002-1909-6343}
\par}
\cmsinstitute{INFN Laboratori Nazionali di Frascati, Frascati, Italy}
{\tolerance=6000
L.~Benussi\cmsorcid{0000-0002-2363-8889}, S.~Bianco\cmsorcid{0000-0002-8300-4124}, S.~Meola\cmsAuthorMark{52}\cmsorcid{0000-0002-8233-7277}, D.~Piccolo\cmsorcid{0000-0001-5404-543X}
\par}
\cmsinstitute{INFN Sezione di Genova$^{a}$, Universit\`{a} di Genova$^{b}$, Genova, Italy}
{\tolerance=6000
P.~Chatagnon$^{a}$\cmsorcid{0000-0002-4705-9582}, F.~Ferro$^{a}$\cmsorcid{0000-0002-7663-0805}, E.~Robutti$^{a}$\cmsorcid{0000-0001-9038-4500}, S.~Tosi$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-7275-9193}
\par}
\cmsinstitute{INFN Sezione di Milano-Bicocca$^{a}$, Universit\`{a} di Milano-Bicocca$^{b}$, Milano, Italy}
{\tolerance=6000
A.~Benaglia$^{a}$\cmsorcid{0000-0003-1124-8450}, G.~Boldrini$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-5490-605X}, F.~Brivio$^{a}$\cmsorcid{0000-0001-9523-6451}, F.~Cetorelli$^{a}$\cmsorcid{0000-0002-3061-1553}, F.~De~Guio$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-5927-8865}, M.E.~Dinardo$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-8575-7250}, P.~Dini$^{a}$\cmsorcid{0000-0001-7375-4899}, S.~Gennai$^{a}$\cmsorcid{0000-0001-5269-8517}, R.~Gerosa$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-8359-3734}, A.~Ghezzi$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-8184-7953}, P.~Govoni$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-0227-1301}, L.~Guzzi$^{a}$\cmsorcid{0000-0002-3086-8260}, M.T.~Lucchini$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-7497-7450}, M.~Malberti$^{a}$\cmsorcid{0000-0001-6794-8419}, S.~Malvezzi$^{a}$\cmsorcid{0000-0002-0218-4910}, A.~Massironi$^{a}$\cmsorcid{0000-0002-0782-0883}, D.~Menasce$^{a}$\cmsorcid{0000-0002-9918-1686}, L.~Moroni$^{a}$\cmsorcid{0000-0002-8387-762X}, M.~Paganoni$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-2461-275X}, D.~Pedrini$^{a}$\cmsorcid{0000-0003-2414-4175}, B.S.~Pinolini$^{a}$, S.~Ragazzi$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-8219-2074}, T.~Tabarelli~de~Fatis$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-6262-4685}, D.~Zuolo$^{a}$\cmsorcid{0000-0003-3072-1020}
\par}
\cmsinstitute{INFN Sezione di Napoli$^{a}$, Universit\`{a} di Napoli 'Federico II'$^{b}$, Napoli, Italy; Universit\`{a} della Basilicata$^{c}$, Potenza, Italy; Universit\`{a} G. Marconi$^{d}$, Roma, Italy}
{\tolerance=6000
S.~Buontempo$^{a}$\cmsorcid{0000-0001-9526-556X}, A.~Cagnotta$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-8801-9894}, F.~Carnevali$^{a}$$^{, }$$^{b}$, N.~Cavallo$^{a}$$^{, }$$^{c}$\cmsorcid{0000-0003-1327-9058}, A.~De~Iorio$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-9258-1345}, F.~Fabozzi$^{a}$$^{, }$$^{c}$\cmsorcid{0000-0001-9821-4151}, A.O.M.~Iorio$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-3798-1135}, L.~Lista$^{a}$$^{, }$$^{b}$$^{, }$\cmsAuthorMark{53}\cmsorcid{0000-0001-6471-5492}, P.~Paolucci$^{a}$$^{, }$\cmsAuthorMark{32}\cmsorcid{0000-0002-8773-4781}, B.~Rossi$^{a}$\cmsorcid{0000-0002-0807-8772}, C.~Sciacca$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-8412-4072}
\par}
\cmsinstitute{INFN Sezione di Padova$^{a}$, Universit\`{a} di Padova$^{b}$, Padova, Italy; Universit\`{a} di Trento$^{c}$, Trento, Italy}
{\tolerance=6000
R.~Ardino$^{a}$\cmsorcid{0000-0001-8348-2962}, P.~Azzi$^{a}$\cmsorcid{0000-0002-3129-828X}, N.~Bacchetta$^{a}$$^{, }$\cmsAuthorMark{54}\cmsorcid{0000-0002-2205-5737}, D.~Bisello$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-2359-8477}, P.~Bortignon$^{a}$\cmsorcid{0000-0002-5360-1454}, A.~Bragagnolo$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-3474-2099}, R.~Carlin$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-7915-1650}, P.~Checchia$^{a}$\cmsorcid{0000-0002-8312-1531}, T.~Dorigo$^{a}$\cmsorcid{0000-0002-1659-8727}, F.~Gasparini$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-1315-563X}, U.~Gasparini$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-7253-2669}, G.~Grosso$^{a}$, L.~Layer$^{a}$$^{, }$\cmsAuthorMark{55}, E.~Lusiani$^{a}$\cmsorcid{0000-0001-8791-7978}, M.~Margoni$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-1797-4330}, A.T.~Meneguzzo$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-5861-8140}, M.~Migliorini$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-5441-7755}, J.~Pazzini$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-1118-6205}, P.~Ronchese$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-7002-2051}, R.~Rossin$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-3466-7500}, F.~Simonetto$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-8279-2464}, G.~Strong$^{a}$\cmsorcid{0000-0002-4640-6108}, M.~Tosi$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-4050-1769}, A.~Triossi$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-5140-9154}, S.~Ventura$^{a}$\cmsorcid{0000-0002-8938-2193}, H.~Yarar$^{a}$$^{, }$$^{b}$, M.~Zanetti$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-4281-4582}, P.~Zotto$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-3953-5996}, A.~Zucchetta$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-0380-1172}, G.~Zumerle$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-3075-2679}
\par}
\cmsinstitute{INFN Sezione di Pavia$^{a}$, Universit\`{a} di Pavia$^{b}$, Pavia, Italy}
{\tolerance=6000
S.~Abu~Zeid$^{a}$$^{, }$\cmsAuthorMark{56}\cmsorcid{0000-0002-0820-0483}, C.~Aim\`{e}$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-0449-4717}, A.~Braghieri$^{a}$\cmsorcid{0000-0002-9606-5604}, S.~Calzaferri$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-1162-2505}, D.~Fiorina$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-7104-257X}, P.~Montagna$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-9647-9420}, V.~Re$^{a}$\cmsorcid{0000-0003-0697-3420}, C.~Riccardi$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-0165-3962}, P.~Salvini$^{a}$\cmsorcid{0000-0001-9207-7256}, I.~Vai$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-0037-5032}, P.~Vitulo$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-9247-7778}
\par}
\cmsinstitute{INFN Sezione di Perugia$^{a}$, Universit\`{a} di Perugia$^{b}$, Perugia, Italy}
{\tolerance=6000
S.~Ajmal$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-2726-2858}, P.~Asenov$^{a}$$^{, }$\cmsAuthorMark{57}\cmsorcid{0000-0003-2379-9903}, G.M.~Bilei$^{a}$\cmsorcid{0000-0002-4159-9123}, D.~Ciangottini$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-0843-4108}, L.~Fan\`{o}$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-9007-629X}, M.~Magherini$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-4108-3925}, G.~Mantovani$^{a}$$^{, }$$^{b}$, V.~Mariani$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-7108-8116}, M.~Menichelli$^{a}$\cmsorcid{0000-0002-9004-735X}, F.~Moscatelli$^{a}$$^{, }$\cmsAuthorMark{57}\cmsorcid{0000-0002-7676-3106}, A.~Rossi$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-2031-2955}, A.~Santocchia$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-9770-2249}, D.~Spiga$^{a}$\cmsorcid{0000-0002-2991-6384}, T.~Tedeschi$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-7125-2905}
\par}
\cmsinstitute{INFN Sezione di Pisa$^{a}$, Universit\`{a} di Pisa$^{b}$, Scuola Normale Superiore di Pisa$^{c}$, Pisa, Italy; Universit\`{a} di Siena$^{d}$, Siena, Italy}
{\tolerance=6000
P.~Azzurri$^{a}$\cmsorcid{0000-0002-1717-5654}, G.~Bagliesi$^{a}$\cmsorcid{0000-0003-4298-1620}, R.~Bhattacharya$^{a}$\cmsorcid{0000-0002-7575-8639}, L.~Bianchini$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-6598-6865}, T.~Boccali$^{a}$\cmsorcid{0000-0002-9930-9299}, E.~Bossini$^{a}$\cmsorcid{0000-0002-2303-2588}, D.~Bruschini$^{a}$$^{, }$$^{c}$\cmsorcid{0000-0001-7248-2967}, R.~Castaldi$^{a}$\cmsorcid{0000-0003-0146-845X}, M.A.~Ciocci$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-0002-5462}, M.~Cipriani$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-0151-4439}, V.~D'Amante$^{a}$$^{, }$$^{d}$\cmsorcid{0000-0002-7342-2592}, R.~Dell'Orso$^{a}$\cmsorcid{0000-0003-1414-9343}, S.~Donato$^{a}$\cmsorcid{0000-0001-7646-4977}, A.~Giassi$^{a}$\cmsorcid{0000-0001-9428-2296}, F.~Ligabue$^{a}$$^{, }$$^{c}$\cmsorcid{0000-0002-1549-7107}, D.~Matos~Figueiredo$^{a}$\cmsorcid{0000-0003-2514-6930}, A.~Messineo$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-7551-5613}, M.~Musich$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-7938-5684}, F.~Palla$^{a}$\cmsorcid{0000-0002-6361-438X}, A.~Rizzi$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-4543-2718}, G.~Rolandi$^{a}$$^{, }$$^{c}$\cmsorcid{0000-0002-0635-274X}, S.~Roy~Chowdhury$^{a}$\cmsorcid{0000-0001-5742-5593}, T.~Sarkar$^{a}$\cmsorcid{0000-0003-0582-4167}, A.~Scribano$^{a}$\cmsorcid{0000-0002-4338-6332}, P.~Spagnolo$^{a}$\cmsorcid{0000-0001-7962-5203}, R.~Tenchini$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-2574-4383}, G.~Tonelli$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-2606-9156}, N.~Turini$^{a}$$^{, }$$^{d}$\cmsorcid{0000-0002-9395-5230}, A.~Venturi$^{a}$\cmsorcid{0000-0002-0249-4142}, P.G.~Verdini$^{a}$\cmsorcid{0000-0002-0042-9507}
\par}
\cmsinstitute{INFN Sezione di Roma$^{a}$, Sapienza Universit\`{a} di Roma$^{b}$, Roma, Italy}
{\tolerance=6000
P.~Barria$^{a}$\cmsorcid{0000-0002-3924-7380}, M.~Campana$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-5425-723X}, F.~Cavallari$^{a}$\cmsorcid{0000-0002-1061-3877}, L.~Cunqueiro~Mendez$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-6764-5370}, D.~Del~Re$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-0870-5796}, E.~Di~Marco$^{a}$\cmsorcid{0000-0002-5920-2438}, M.~Diemoz$^{a}$\cmsorcid{0000-0002-3810-8530}, F.~Errico$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-8199-370X}, E.~Longo$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-6238-6787}, P.~Meridiani$^{a}$\cmsorcid{0000-0002-8480-2259}, J.~Mijuskovic$^{a}$$^{, }$$^{b}$\cmsorcid{0009-0009-1589-9980}, G.~Organtini$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-3229-0781}, F.~Pandolfi$^{a}$\cmsorcid{0000-0001-8713-3874}, R.~Paramatti$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-0080-9550}, C.~Quaranta$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-0042-6891}, S.~Rahatlou$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-9794-3360}, C.~Rovelli$^{a}$\cmsorcid{0000-0003-2173-7530}, F.~Santanastasio$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-2505-8359}, L.~Soffi$^{a}$\cmsorcid{0000-0003-2532-9876}
\par}
\cmsinstitute{INFN Sezione di Torino$^{a}$, Universit\`{a} di Torino$^{b}$, Torino, Italy; Universit\`{a} del Piemonte Orientale$^{c}$, Novara, Italy}
{\tolerance=6000
N.~Amapane$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-9449-2509}, R.~Arcidiacono$^{a}$$^{, }$$^{c}$\cmsorcid{0000-0001-5904-142X}, S.~Argiro$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-2150-3750}, M.~Arneodo$^{a}$$^{, }$$^{c}$\cmsorcid{0000-0002-7790-7132}, N.~Bartosik$^{a}$\cmsorcid{0000-0002-7196-2237}, R.~Bellan$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-2539-2376}, A.~Bellora$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-2753-5473}, C.~Biino$^{a}$\cmsorcid{0000-0002-1397-7246}, N.~Cartiglia$^{a}$\cmsorcid{0000-0002-0548-9189}, M.~Costa$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-0156-0790}, R.~Covarelli$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-1216-5235}, N.~Demaria$^{a}$\cmsorcid{0000-0003-0743-9465}, L.~Finco$^{a}$\cmsorcid{0000-0002-2630-5465}, M.~Grippo$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-0770-269X}, B.~Kiani$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-1202-7652}, F.~Legger$^{a}$\cmsorcid{0000-0003-1400-0709}, F.~Luongo$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-2743-4119}, C.~Mariotti$^{a}$\cmsorcid{0000-0002-6864-3294}, S.~Maselli$^{a}$\cmsorcid{0000-0001-9871-7859}, A.~Mecca$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-2209-2527}, E.~Migliore$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-2271-5192}, M.~Monteno$^{a}$\cmsorcid{0000-0002-3521-6333}, R.~Mulargia$^{a}$\cmsorcid{0000-0003-2437-013X}, M.M.~Obertino$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-8781-8192}, G.~Ortona$^{a}$\cmsorcid{0000-0001-8411-2971}, L.~Pacher$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-1288-4838}, N.~Pastrone$^{a}$\cmsorcid{0000-0001-7291-1979}, M.~Pelliccioni$^{a}$\cmsorcid{0000-0003-4728-6678}, M.~Ruspa$^{a}$$^{, }$$^{c}$\cmsorcid{0000-0002-7655-3475}, F.~Siviero$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-4427-4076}, V.~Sola$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-6288-951X}, A.~Solano$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-2971-8214}, D.~Soldi$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-9059-4831}, A.~Staiano$^{a}$\cmsorcid{0000-0003-1803-624X}, C.~Tarricone$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0001-6233-0513}, D.~Trocino$^{a}$\cmsorcid{0000-0002-2830-5872}, G.~Umoret$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-6674-7874}, E.~Vlasov$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-8628-2090}
\par}
\cmsinstitute{INFN Sezione di Trieste$^{a}$, Universit\`{a} di Trieste$^{b}$, Trieste, Italy}
{\tolerance=6000
S.~Belforte$^{a}$\cmsorcid{0000-0001-8443-4460}, V.~Candelise$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-3641-5983}, M.~Casarsa$^{a}$\cmsorcid{0000-0002-1353-8964}, F.~Cossutti$^{a}$\cmsorcid{0000-0001-5672-214X}, K.~De~Leo$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0002-8908-409X}, G.~Della~Ricca$^{a}$$^{, }$$^{b}$\cmsorcid{0000-0003-2831-6982}
\par}
\cmsinstitute{Kyungpook National University, Daegu, Korea}
{\tolerance=6000
S.~Dogra\cmsorcid{0000-0002-0812-0758}, J.~Hong\cmsorcid{0000-0002-9463-4922}, C.~Huh\cmsorcid{0000-0002-8513-2824}, B.~Kim\cmsorcid{0000-0002-9539-6815}, D.H.~Kim\cmsorcid{0000-0002-9023-6847}, J.~Kim, H.~Lee, S.W.~Lee\cmsorcid{0000-0002-1028-3468}, C.S.~Moon\cmsorcid{0000-0001-8229-7829}, Y.D.~Oh\cmsorcid{0000-0002-7219-9931}, M.S.~Ryu\cmsorcid{0000-0002-1855-180X}, S.~Sekmen\cmsorcid{0000-0003-1726-5681}, Y.C.~Yang\cmsorcid{0000-0003-1009-4621}
\par}
\cmsinstitute{Department of Mathematics and Physics - GWNU, Gangneung, Korea}
{\tolerance=6000
M.S.~Kim\cmsorcid{0000-0003-0392-8691}
\par}
\cmsinstitute{Chonnam National University, Institute for Universe and Elementary Particles, Kwangju, Korea}
{\tolerance=6000
G.~Bak\cmsorcid{0000-0002-0095-8185}, P.~Gwak\cmsorcid{0009-0009-7347-1480}, H.~Kim\cmsorcid{0000-0001-8019-9387}, D.H.~Moon\cmsorcid{0000-0002-5628-9187}
\par}
\cmsinstitute{Hanyang University, Seoul, Korea}
{\tolerance=6000
E.~Asilar\cmsorcid{0000-0001-5680-599X}, D.~Kim\cmsorcid{0000-0002-8336-9182}, T.J.~Kim\cmsorcid{0000-0001-8336-2434}, J.A.~Merlin
\par}
\cmsinstitute{Korea University, Seoul, Korea}
{\tolerance=6000
S.~Choi\cmsorcid{0000-0001-6225-9876}, S.~Han, B.~Hong\cmsorcid{0000-0002-2259-9929}, K.~Lee, K.S.~Lee\cmsorcid{0000-0002-3680-7039}, S.~Lee\cmsorcid{0000-0001-9257-9643}, J.~Park, S.K.~Park, J.~Yoo\cmsorcid{0000-0003-0463-3043}
\par}
\cmsinstitute{Kyung Hee University, Department of Physics, Seoul, Korea}
{\tolerance=6000
J.~Goh\cmsorcid{0000-0002-1129-2083}
\par}
\cmsinstitute{Sejong University, Seoul, Korea}
{\tolerance=6000
H.~S.~Kim\cmsorcid{0000-0002-6543-9191}, Y.~Kim, S.~Lee
\par}
\cmsinstitute{Seoul National University, Seoul, Korea}
{\tolerance=6000
J.~Almond, J.H.~Bhyun, J.~Choi\cmsorcid{0000-0002-2483-5104}, W.~Jun\cmsorcid{0009-0001-5122-4552}, J.~Kim\cmsorcid{0000-0001-9876-6642}, J.S.~Kim, S.~Ko\cmsorcid{0000-0003-4377-9969}, H.~Kwon\cmsorcid{0009-0002-5165-5018}, H.~Lee\cmsorcid{0000-0002-1138-3700}, J.~Lee\cmsorcid{0000-0001-6753-3731}, J.~Lee\cmsorcid{0000-0002-5351-7201}, B.H.~Oh\cmsorcid{0000-0002-9539-7789}, S.B.~Oh\cmsorcid{0000-0003-0710-4956}, H.~Seo\cmsorcid{0000-0002-3932-0605}, U.K.~Yang, I.~Yoon\cmsorcid{0000-0002-3491-8026}
\par}
\cmsinstitute{University of Seoul, Seoul, Korea}
{\tolerance=6000
W.~Jang\cmsorcid{0000-0002-1571-9072}, D.Y.~Kang, Y.~Kang\cmsorcid{0000-0001-6079-3434}, S.~Kim\cmsorcid{0000-0002-8015-7379}, B.~Ko, J.S.H.~Lee\cmsorcid{0000-0002-2153-1519}, Y.~Lee\cmsorcid{0000-0001-5572-5947}, I.C.~Park\cmsorcid{0000-0003-4510-6776}, Y.~Roh, I.J.~Watson\cmsorcid{0000-0003-2141-3413}, S.~Yang\cmsorcid{0000-0001-6905-6553}
\par}
\cmsinstitute{Yonsei University, Department of Physics, Seoul, Korea}
{\tolerance=6000
S.~Ha\cmsorcid{0000-0003-2538-1551}, H.D.~Yoo\cmsorcid{0000-0002-3892-3500}
\par}
\cmsinstitute{Sungkyunkwan University, Suwon, Korea}
{\tolerance=6000
M.~Choi\cmsorcid{0000-0002-4811-626X}, M.R.~Kim\cmsorcid{0000-0002-2289-2527}, H.~Lee, Y.~Lee\cmsorcid{0000-0001-6954-9964}, I.~Yu\cmsorcid{0000-0003-1567-5548}
\par}
\cmsinstitute{College of Engineering and Technology, American University of the Middle East (AUM), Dasman, Kuwait}
{\tolerance=6000
T.~Beyrouthy, Y.~Maghrbi\cmsorcid{0000-0002-4960-7458}
\par}
\cmsinstitute{Riga Technical University, Riga, Latvia}
{\tolerance=6000
K.~Dreimanis\cmsorcid{0000-0003-0972-5641}, A.~Gaile\cmsorcid{0000-0003-1350-3523}, G.~Pikurs, A.~Potrebko\cmsorcid{0000-0002-3776-8270}, M.~Seidel\cmsorcid{0000-0003-3550-6151}, V.~Veckalns\cmsAuthorMark{58}\cmsorcid{0000-0003-3676-9711}
\par}
\cmsinstitute{University of Latvia (LU), Riga, Latvia}
{\tolerance=6000
N.R.~Strautnieks\cmsorcid{0000-0003-4540-9048}
\par}
\cmsinstitute{Vilnius University, Vilnius, Lithuania}
{\tolerance=6000
M.~Ambrozas\cmsorcid{0000-0003-2449-0158}, A.~Juodagalvis\cmsorcid{0000-0002-1501-3328}, A.~Rinkevicius\cmsorcid{0000-0002-7510-255X}, G.~Tamulaitis\cmsorcid{0000-0002-2913-9634}
\par}
\cmsinstitute{National Centre for Particle Physics, Universiti Malaya, Kuala Lumpur, Malaysia}
{\tolerance=6000
N.~Bin~Norjoharuddeen\cmsorcid{0000-0002-8818-7476}, I.~Yusuff\cmsAuthorMark{59}\cmsorcid{0000-0003-2786-0732}, Z.~Zolkapli
\par}
\cmsinstitute{Universidad de Sonora (UNISON), Hermosillo, Mexico}
{\tolerance=6000
J.F.~Benitez\cmsorcid{0000-0002-2633-6712}, A.~Castaneda~Hernandez\cmsorcid{0000-0003-4766-1546}, H.A.~Encinas~Acosta, L.G.~Gallegos~Mar\'{i}\~{n}ez, M.~Le\'{o}n~Coello\cmsorcid{0000-0002-3761-911X}, J.A.~Murillo~Quijada\cmsorcid{0000-0003-4933-2092}, A.~Sehrawat\cmsorcid{0000-0002-6816-7814}, L.~Valencia~Palomo\cmsorcid{0000-0002-8736-440X}
\par}
\cmsinstitute{Centro de Investigacion y de Estudios Avanzados del IPN, Mexico City, Mexico}
{\tolerance=6000
G.~Ayala\cmsorcid{0000-0002-8294-8692}, H.~Castilla-Valdez\cmsorcid{0009-0005-9590-9958}, E.~De~La~Cruz-Burelo\cmsorcid{0000-0002-7469-6974}, I.~Heredia-De~La~Cruz\cmsAuthorMark{60}\cmsorcid{0000-0002-8133-6467}, R.~Lopez-Fernandez\cmsorcid{0000-0002-2389-4831}, C.A.~Mondragon~Herrera, A.~S\'{a}nchez~Hern\'{a}ndez\cmsorcid{0000-0001-9548-0358}
\par}
\cmsinstitute{Universidad Iberoamericana, Mexico City, Mexico}
{\tolerance=6000
C.~Oropeza~Barrera\cmsorcid{0000-0001-9724-0016}, M.~Ram\'{i}rez~Garc\'{i}a\cmsorcid{0000-0002-4564-3822}
\par}
\cmsinstitute{Benemerita Universidad Autonoma de Puebla, Puebla, Mexico}
{\tolerance=6000
I.~Bautista\cmsorcid{0000-0001-5873-3088}, I.~Pedraza\cmsorcid{0000-0002-2669-4659}, H.A.~Salazar~Ibarguen\cmsorcid{0000-0003-4556-7302}, C.~Uribe~Estrada\cmsorcid{0000-0002-2425-7340}
\par}
\cmsinstitute{University of Montenegro, Podgorica, Montenegro}
{\tolerance=6000
I.~Bubanja, N.~Raicevic\cmsorcid{0000-0002-2386-2290}
\par}
\cmsinstitute{University of Canterbury, Christchurch, New Zealand}
{\tolerance=6000
P.H.~Butler\cmsorcid{0000-0001-9878-2140}
\par}
\cmsinstitute{National Centre for Physics, Quaid-I-Azam University, Islamabad, Pakistan}
{\tolerance=6000
A.~Ahmad\cmsorcid{0000-0002-4770-1897}, M.I.~Asghar, A.~Awais\cmsorcid{0000-0003-3563-257X}, M.I.M.~Awan, H.R.~Hoorani\cmsorcid{0000-0002-0088-5043}, W.A.~Khan\cmsorcid{0000-0003-0488-0941}
\par}
\cmsinstitute{AGH University of Science and Technology Faculty of Computer Science, Electronics and Telecommunications, Krakow, Poland}
{\tolerance=6000
V.~Avati, L.~Grzanka\cmsorcid{0000-0002-3599-854X}, M.~Malawski\cmsorcid{0000-0001-6005-0243}
\par}
\cmsinstitute{National Centre for Nuclear Research, Swierk, Poland}
{\tolerance=6000
H.~Bialkowska\cmsorcid{0000-0002-5956-6258}, M.~Bluj\cmsorcid{0000-0003-1229-1442}, B.~Boimska\cmsorcid{0000-0002-4200-1541}, M.~G\'{o}rski\cmsorcid{0000-0003-2146-187X}, M.~Kazana\cmsorcid{0000-0002-7821-3036}, M.~Szleper\cmsorcid{0000-0002-1697-004X}, P.~Zalewski\cmsorcid{0000-0003-4429-2888}
\par}
\cmsinstitute{Institute of Experimental Physics, Faculty of Physics, University of Warsaw, Warsaw, Poland}
{\tolerance=6000
K.~Bunkowski\cmsorcid{0000-0001-6371-9336}, K.~Doroba\cmsorcid{0000-0002-7818-2364}, A.~Kalinowski\cmsorcid{0000-0002-1280-5493}, M.~Konecki\cmsorcid{0000-0001-9482-4841}, J.~Krolikowski\cmsorcid{0000-0002-3055-0236}, A.~Muhammad\cmsorcid{0000-0002-7535-7149}
\par}
\cmsinstitute{Laborat\'{o}rio de Instrumenta\c{c}\~{a}o e F\'{i}sica Experimental de Part\'{i}culas, Lisboa, Portugal}
{\tolerance=6000
M.~Araujo\cmsorcid{0000-0002-8152-3756}, D.~Bastos\cmsorcid{0000-0002-7032-2481}, C.~Beir\~{a}o~Da~Cruz~E~Silva\cmsorcid{0000-0002-1231-3819}, A.~Boletti\cmsorcid{0000-0003-3288-7737}, M.~Bozzo\cmsorcid{0000-0002-1715-0457}, T.~Camporesi\cmsorcid{0000-0001-5066-1876}, G.~Da~Molin\cmsorcid{0000-0003-2163-5569}, P.~Faccioli\cmsorcid{0000-0003-1849-6692}, M.~Gallinaro\cmsorcid{0000-0003-1261-2277}, J.~Hollar\cmsorcid{0000-0002-8664-0134}, N.~Leonardo\cmsorcid{0000-0002-9746-4594}, T.~Niknejad\cmsorcid{0000-0003-3276-9482}, A.~Petrilli\cmsorcid{0000-0003-0887-1882}, M.~Pisano\cmsorcid{0000-0002-0264-7217}, J.~Seixas\cmsorcid{0000-0002-7531-0842}, J.~Varela\cmsorcid{0000-0003-2613-3146}, J.W.~Wulff
\par}
\cmsinstitute{Faculty of Physics, University of Belgrade, Belgrade, Serbia}
{\tolerance=6000
P.~Adzic\cmsorcid{0000-0002-5862-7397}, P.~Milenovic\cmsorcid{0000-0001-7132-3550}
\par}
\cmsinstitute{VINCA Institute of Nuclear Sciences, University of Belgrade, Belgrade, Serbia}
{\tolerance=6000
M.~Dordevic\cmsorcid{0000-0002-8407-3236}, J.~Milosevic\cmsorcid{0000-0001-8486-4604}, V.~Rekovic
\par}
\cmsinstitute{Centro de Investigaciones Energ\'{e}ticas Medioambientales y Tecnol\'{o}gicas (CIEMAT), Madrid, Spain}
{\tolerance=6000
M.~Aguilar-Benitez, J.~Alcaraz~Maestre\cmsorcid{0000-0003-0914-7474}, Cristina~F.~Bedoya\cmsorcid{0000-0001-8057-9152}, M.~Cepeda\cmsorcid{0000-0002-6076-4083}, M.~Cerrada\cmsorcid{0000-0003-0112-1691}, N.~Colino\cmsorcid{0000-0002-3656-0259}, B.~De~La~Cruz\cmsorcid{0000-0001-9057-5614}, A.~Delgado~Peris\cmsorcid{0000-0002-8511-7958}, D.~Fern\'{a}ndez~Del~Val\cmsorcid{0000-0003-2346-1590}, J.P.~Fern\'{a}ndez~Ramos\cmsorcid{0000-0002-0122-313X}, J.~Flix\cmsorcid{0000-0003-2688-8047}, M.C.~Fouz\cmsorcid{0000-0003-2950-976X}, O.~Gonzalez~Lopez\cmsorcid{0000-0002-4532-6464}, S.~Goy~Lopez\cmsorcid{0000-0001-6508-5090}, J.M.~Hernandez\cmsorcid{0000-0001-6436-7547}, M.I.~Josa\cmsorcid{0000-0002-4985-6964}, J.~Le\'{o}n~Holgado\cmsorcid{0000-0002-4156-6460}, D.~Moran\cmsorcid{0000-0002-1941-9333}, C.~M.~Morcillo~Perez\cmsorcid{0000-0001-9634-848X}, \'{A}.~Navarro~Tobar\cmsorcid{0000-0003-3606-1780}, C.~Perez~Dengra\cmsorcid{0000-0003-2821-4249}, A.~P\'{e}rez-Calero~Yzquierdo\cmsorcid{0000-0003-3036-7965}, J.~Puerta~Pelayo\cmsorcid{0000-0001-7390-1457}, I.~Redondo\cmsorcid{0000-0003-3737-4121}, D.D.~Redondo~Ferrero\cmsorcid{0000-0002-3463-0559}, L.~Romero, S.~S\'{a}nchez~Navas\cmsorcid{0000-0001-6129-9059}, L.~Urda~G\'{o}mez\cmsorcid{0000-0002-7865-5010}, J.~Vazquez~Escobar\cmsorcid{0000-0002-7533-2283}, C.~Willmott
\par}
\cmsinstitute{Universidad Aut\'{o}noma de Madrid, Madrid, Spain}
{\tolerance=6000
J.F.~de~Troc\'{o}niz\cmsorcid{0000-0002-0798-9806}
\par}
\cmsinstitute{Universidad de Oviedo, Instituto Universitario de Ciencias y Tecnolog\'{i}as Espaciales de Asturias (ICTEA), Oviedo, Spain}
{\tolerance=6000
B.~Alvarez~Gonzalez\cmsorcid{0000-0001-7767-4810}, J.~Cuevas\cmsorcid{0000-0001-5080-0821}, J.~Fernandez~Menendez\cmsorcid{0000-0002-5213-3708}, S.~Folgueras\cmsorcid{0000-0001-7191-1125}, I.~Gonzalez~Caballero\cmsorcid{0000-0002-8087-3199}, J.R.~Gonz\'{a}lez~Fern\'{a}ndez\cmsorcid{0000-0002-4825-8188}, E.~Palencia~Cortezon\cmsorcid{0000-0001-8264-0287}, C.~Ram\'{o}n~\'{A}lvarez\cmsorcid{0000-0003-1175-0002}, V.~Rodr\'{i}guez~Bouza\cmsorcid{0000-0002-7225-7310}, A.~Soto~Rodr\'{i}guez\cmsorcid{0000-0002-2993-8663}, A.~Trapote\cmsorcid{0000-0002-4030-2551}, C.~Vico~Villalba\cmsorcid{0000-0002-1905-1874}, P.~Vischia\cmsorcid{0000-0002-7088-8557}
\par}
\cmsinstitute{Instituto de F\'{i}sica de Cantabria (IFCA), CSIC-Universidad de Cantabria, Santander, Spain}
{\tolerance=6000
S.~Bhowmik\cmsorcid{0000-0003-1260-973X}, S.~Blanco~Fern\'{a}ndez\cmsorcid{0000-0001-7301-0670}, J.A.~Brochero~Cifuentes\cmsorcid{0000-0003-2093-7856}, I.J.~Cabrillo\cmsorcid{0000-0002-0367-4022}, A.~Calderon\cmsorcid{0000-0002-7205-2040}, J.~Duarte~Campderros\cmsorcid{0000-0003-0687-5214}, M.~Fernandez\cmsorcid{0000-0002-4824-1087}, C.~Fernandez~Madrazo\cmsorcid{0000-0001-9748-4336}, G.~Gomez\cmsorcid{0000-0002-1077-6553}, C.~Lasaosa~Garc\'{i}a\cmsorcid{0000-0003-2726-7111}, C.~Martinez~Rivero\cmsorcid{0000-0002-3224-956X}, P.~Martinez~Ruiz~del~Arbol\cmsorcid{0000-0002-7737-5121}, F.~Matorras\cmsorcid{0000-0003-4295-5668}, P.~Matorras~Cuevas\cmsorcid{0000-0001-7481-7273}, E.~Navarrete~Ramos\cmsorcid{0000-0002-5180-4020}, J.~Piedra~Gomez\cmsorcid{0000-0002-9157-1700}, L.~Scodellaro\cmsorcid{0000-0002-4974-8330}, I.~Vila\cmsorcid{0000-0002-6797-7209}, J.M.~Vizan~Garcia\cmsorcid{0000-0002-6823-8854}
\par}
\cmsinstitute{University of Colombo, Colombo, Sri Lanka}
{\tolerance=6000
M.K.~Jayananda\cmsorcid{0000-0002-7577-310X}, B.~Kailasapathy\cmsAuthorMark{61}\cmsorcid{0000-0003-2424-1303}, D.U.J.~Sonnadara\cmsorcid{0000-0001-7862-2537}, D.D.C.~Wickramarathna\cmsorcid{0000-0002-6941-8478}
\par}
\cmsinstitute{University of Ruhuna, Department of Physics, Matara, Sri Lanka}
{\tolerance=6000
W.G.D.~Dharmaratna\cmsorcid{0000-0002-6366-837X}, K.~Liyanage\cmsorcid{0000-0002-3792-7665}, N.~Perera\cmsorcid{0000-0002-4747-9106}, N.~Wickramage\cmsorcid{0000-0001-7760-3537}
\par}
\cmsinstitute{CERN, European Organization for Nuclear Research, Geneva, Switzerland}
{\tolerance=6000
D.~Abbaneo\cmsorcid{0000-0001-9416-1742}, C.~Amendola\cmsorcid{0000-0002-4359-836X}, E.~Auffray\cmsorcid{0000-0001-8540-1097}, G.~Auzinger\cmsorcid{0000-0001-7077-8262}, J.~Baechler, D.~Barney\cmsorcid{0000-0002-4927-4921}, A.~Berm\'{u}dez~Mart\'{i}nez\cmsorcid{0000-0001-8822-4727}, M.~Bianco\cmsorcid{0000-0002-8336-3282}, B.~Bilin\cmsorcid{0000-0003-1439-7128}, A.A.~Bin~Anuar\cmsorcid{0000-0002-2988-9830}, A.~Bocci\cmsorcid{0000-0002-6515-5666}, E.~Brondolin\cmsorcid{0000-0001-5420-586X}, C.~Caillol\cmsorcid{0000-0002-5642-3040}, G.~Cerminara\cmsorcid{0000-0002-2897-5753}, N.~Chernyavskaya\cmsorcid{0000-0002-2264-2229}, D.~d'Enterria\cmsorcid{0000-0002-5754-4303}, A.~Dabrowski\cmsorcid{0000-0003-2570-9676}, A.~David\cmsorcid{0000-0001-5854-7699}, A.~De~Roeck\cmsorcid{0000-0002-9228-5271}, M.M.~Defranchis\cmsorcid{0000-0001-9573-3714}, M.~Deile\cmsorcid{0000-0001-5085-7270}, M.~Dobson\cmsorcid{0009-0007-5021-3230}, F.~Fallavollita\cmsAuthorMark{62}, L.~Forthomme\cmsorcid{0000-0002-3302-336X}, G.~Franzoni\cmsorcid{0000-0001-9179-4253}, W.~Funk\cmsorcid{0000-0003-0422-6739}, S.~Giani, D.~Gigi, K.~Gill\cmsorcid{0009-0001-9331-5145}, F.~Glege\cmsorcid{0000-0002-4526-2149}, L.~Gouskos\cmsorcid{0000-0002-9547-7471}, M.~Haranko\cmsorcid{0000-0002-9376-9235}, J.~Hegeman\cmsorcid{0000-0002-2938-2263}, B.~Huber, V.~Innocente\cmsorcid{0000-0003-3209-2088}, T.~James\cmsorcid{0000-0002-3727-0202}, P.~Janot\cmsorcid{0000-0001-7339-4272}, S.~Laurila\cmsorcid{0000-0001-7507-8636}, P.~Lecoq\cmsorcid{0000-0002-3198-0115}, E.~Leutgeb\cmsorcid{0000-0003-4838-3306}, C.~Louren\c{c}o\cmsorcid{0000-0003-0885-6711}, B.~Maier\cmsorcid{0000-0001-5270-7540}, L.~Malgeri\cmsorcid{0000-0002-0113-7389}, M.~Mannelli\cmsorcid{0000-0003-3748-8946}, A.C.~Marini\cmsorcid{0000-0003-2351-0487}, M.~Matthewman, F.~Meijers\cmsorcid{0000-0002-6530-3657}, S.~Mersi\cmsorcid{0000-0003-2155-6692}, E.~Meschi\cmsorcid{0000-0003-4502-6151}, V.~Milosevic\cmsorcid{0000-0002-1173-0696}, F.~Moortgat\cmsorcid{0000-0001-7199-0046}, M.~Mulders\cmsorcid{0000-0001-7432-6634}, S.~Orfanelli, F.~Pantaleo\cmsorcid{0000-0003-3266-4357}, G.~Petrucciani\cmsorcid{0000-0003-0889-4726}, A.~Pfeiffer\cmsorcid{0000-0001-5328-448X}, M.~Pierini\cmsorcid{0000-0003-1939-4268}, D.~Piparo\cmsorcid{0009-0006-6958-3111}, H.~Qu\cmsorcid{0000-0002-0250-8655}, D.~Rabady\cmsorcid{0000-0001-9239-0605}, G.~Reales~Guti\'{e}rrez, M.~Rovere\cmsorcid{0000-0001-8048-1622}, H.~Sakulin\cmsorcid{0000-0003-2181-7258}, S.~Scarfi\cmsorcid{0009-0006-8689-3576}, M.~Selvaggi\cmsorcid{0000-0002-5144-9655}, A.~Sharma\cmsorcid{0000-0002-9860-1650}, K.~Shchelina\cmsorcid{0000-0003-3742-0693}, P.~Silva\cmsorcid{0000-0002-5725-041X}, P.~Sphicas\cmsAuthorMark{63}\cmsorcid{0000-0002-5456-5977}, A.G.~Stahl~Leiton\cmsorcid{0000-0002-5397-252X}, A.~Steen\cmsorcid{0009-0006-4366-3463}, S.~Summers\cmsorcid{0000-0003-4244-2061}, D.~Treille\cmsorcid{0009-0005-5952-9843}, P.~Tropea\cmsorcid{0000-0003-1899-2266}, A.~Tsirou, D.~Walter\cmsorcid{0000-0001-8584-9705}, J.~Wanczyk\cmsAuthorMark{64}\cmsorcid{0000-0002-8562-1863}, K.A.~Wozniak\cmsAuthorMark{65}\cmsorcid{0000-0002-4395-1581}, S.~Wuchterl\cmsorcid{0000-0001-9955-9258}, P.~Zehetner\cmsorcid{0009-0002-0555-4697}, P.~Zejdl\cmsorcid{0000-0001-9554-7815}, W.D.~Zeuner
\par}
\cmsinstitute{Paul Scherrer Institut, Villigen, Switzerland}
{\tolerance=6000
T.~Bevilacqua\cmsAuthorMark{66}\cmsorcid{0000-0001-9791-2353}, L.~Caminada\cmsAuthorMark{66}\cmsorcid{0000-0001-5677-6033}, A.~Ebrahimi\cmsorcid{0000-0003-4472-867X}, W.~Erdmann\cmsorcid{0000-0001-9964-249X}, R.~Horisberger\cmsorcid{0000-0002-5594-1321}, Q.~Ingram\cmsorcid{0000-0002-9576-055X}, H.C.~Kaestli\cmsorcid{0000-0003-1979-7331}, D.~Kotlinski\cmsorcid{0000-0001-5333-4918}, C.~Lange\cmsorcid{0000-0002-3632-3157}, M.~Missiroli\cmsAuthorMark{66}\cmsorcid{0000-0002-1780-1344}, L.~Noehte\cmsAuthorMark{66}\cmsorcid{0000-0001-6125-7203}, T.~Rohe\cmsorcid{0009-0005-6188-7754}
\par}
\cmsinstitute{ETH Zurich - Institute for Particle Physics and Astrophysics (IPA), Zurich, Switzerland}
{\tolerance=6000
T.K.~Aarrestad\cmsorcid{0000-0002-7671-243X}, K.~Androsov\cmsAuthorMark{64}\cmsorcid{0000-0003-2694-6542}, M.~Backhaus\cmsorcid{0000-0002-5888-2304}, A.~Calandri\cmsorcid{0000-0001-7774-0099}, C.~Cazzaniga\cmsorcid{0000-0003-0001-7657}, K.~Datta\cmsorcid{0000-0002-6674-0015}, A.~De~Cosa\cmsorcid{0000-0003-2533-2856}, G.~Dissertori\cmsorcid{0000-0002-4549-2569}, M.~Dittmar, M.~Doneg\`{a}\cmsorcid{0000-0001-9830-0412}, F.~Eble\cmsorcid{0009-0002-0638-3447}, M.~Galli\cmsorcid{0000-0002-9408-4756}, K.~Gedia\cmsorcid{0009-0006-0914-7684}, F.~Glessgen\cmsorcid{0000-0001-5309-1960}, C.~Grab\cmsorcid{0000-0002-6182-3380}, D.~Hits\cmsorcid{0000-0002-3135-6427}, W.~Lustermann\cmsorcid{0000-0003-4970-2217}, A.-M.~Lyon\cmsorcid{0009-0004-1393-6577}, R.A.~Manzoni\cmsorcid{0000-0002-7584-5038}, M.~Marchegiani\cmsorcid{0000-0002-0389-8640}, L.~Marchese\cmsorcid{0000-0001-6627-8716}, C.~Martin~Perez\cmsorcid{0000-0003-1581-6152}, A.~Mascellani\cmsAuthorMark{64}\cmsorcid{0000-0001-6362-5356}, F.~Nessi-Tedaldi\cmsorcid{0000-0002-4721-7966}, F.~Pauss\cmsorcid{0000-0002-3752-4639}, V.~Perovic\cmsorcid{0009-0002-8559-0531}, S.~Pigazzini\cmsorcid{0000-0002-8046-4344}, M.G.~Ratti\cmsorcid{0000-0003-1777-7855}, M.~Reichmann\cmsorcid{0000-0002-6220-5496}, C.~Reissel\cmsorcid{0000-0001-7080-1119}, T.~Reitenspiess\cmsorcid{0000-0002-2249-0835}, B.~Ristic\cmsorcid{0000-0002-8610-1130}, F.~Riti\cmsorcid{0000-0002-1466-9077}, D.~Ruini, D.A.~Sanz~Becerra\cmsorcid{0000-0002-6610-4019}, R.~Seidita\cmsorcid{0000-0002-3533-6191}, J.~Steggemann\cmsAuthorMark{64}\cmsorcid{0000-0003-4420-5510}, D.~Valsecchi\cmsorcid{0000-0001-8587-8266}, R.~Wallny\cmsorcid{0000-0001-8038-1613}
\par}
\cmsinstitute{Universit\"{a}t Z\"{u}rich, Zurich, Switzerland}
{\tolerance=6000
C.~Amsler\cmsAuthorMark{67}\cmsorcid{0000-0002-7695-501X}, P.~B\"{a}rtschi\cmsorcid{0000-0002-8842-6027}, C.~Botta\cmsorcid{0000-0002-8072-795X}, D.~Brzhechko, M.F.~Canelli\cmsorcid{0000-0001-6361-2117}, K.~Cormier\cmsorcid{0000-0001-7873-3579}, R.~Del~Burgo, J.K.~Heikkil\"{a}\cmsorcid{0000-0002-0538-1469}, M.~Huwiler\cmsorcid{0000-0002-9806-5907}, W.~Jin\cmsorcid{0009-0009-8976-7702}, A.~Jofrehei\cmsorcid{0000-0002-8992-5426}, B.~Kilminster\cmsorcid{0000-0002-6657-0407}, S.~Leontsinis\cmsorcid{0000-0002-7561-6091}, S.P.~Liechti\cmsorcid{0000-0002-1192-1628}, A.~Macchiolo\cmsorcid{0000-0003-0199-6957}, P.~Meiring\cmsorcid{0009-0001-9480-4039}, V.M.~Mikuni\cmsorcid{0000-0002-1579-2421}, U.~Molinatti\cmsorcid{0000-0002-9235-3406}, I.~Neutelings\cmsorcid{0009-0002-6473-1403}, A.~Reimers\cmsorcid{0000-0002-9438-2059}, P.~Robmann, S.~Sanchez~Cruz\cmsorcid{0000-0002-9991-195X}, K.~Schweiger\cmsorcid{0000-0002-5846-3919}, M.~Senger\cmsorcid{0000-0002-1992-5711}, Y.~Takahashi\cmsorcid{0000-0001-5184-2265}, R.~Tramontano\cmsorcid{0000-0001-5979-5299}
\par}
\cmsinstitute{National Central University, Chung-Li, Taiwan}
{\tolerance=6000
C.~Adloff\cmsAuthorMark{68}, C.M.~Kuo, W.~Lin, P.K.~Rout\cmsorcid{0000-0001-8149-6180}, P.C.~Tiwari\cmsAuthorMark{42}\cmsorcid{0000-0002-3667-3843}, S.S.~Yu\cmsorcid{0000-0002-6011-8516}
\par}
\cmsinstitute{National Taiwan University (NTU), Taipei, Taiwan}
{\tolerance=6000
L.~Ceard, Y.~Chao\cmsorcid{0000-0002-5976-318X}, K.F.~Chen\cmsorcid{0000-0003-1304-3782}, P.s.~Chen, Z.g.~Chen, W.-S.~Hou\cmsorcid{0000-0002-4260-5118}, T.h.~Hsu, Y.w.~Kao, R.~Khurana, G.~Kole\cmsorcid{0000-0002-3285-1497}, Y.y.~Li\cmsorcid{0000-0003-3598-556X}, R.-S.~Lu\cmsorcid{0000-0001-6828-1695}, E.~Paganis\cmsorcid{0000-0002-1950-8993}, A.~Psallidas, X.f.~Su, J.~Thomas-Wilsker\cmsorcid{0000-0003-1293-4153}, L.s.~Tsai, H.y.~Wu, E.~Yazgan\cmsorcid{0000-0001-5732-7950}
\par}
\cmsinstitute{Chulalongkorn University, Faculty of Science, Department of Physics, Bangkok, Thailand}
{\tolerance=6000
C.~Asawatangtrakuldee\cmsorcid{0000-0003-2234-7219}, N.~Srimanobhas\cmsorcid{0000-0003-3563-2959}, V.~Wachirapusitanand\cmsorcid{0000-0001-8251-5160}
\par}
\cmsinstitute{\c{C}ukurova University, Physics Department, Science and Art Faculty, Adana, Turkey}
{\tolerance=6000
D.~Agyel\cmsorcid{0000-0002-1797-8844}, F.~Boran\cmsorcid{0000-0002-3611-390X}, Z.S.~Demiroglu\cmsorcid{0000-0001-7977-7127}, F.~Dolek\cmsorcid{0000-0001-7092-5517}, I.~Dumanoglu\cmsAuthorMark{69}\cmsorcid{0000-0002-0039-5503}, E.~Eskut\cmsorcid{0000-0001-8328-3314}, Y.~Guler\cmsAuthorMark{70}\cmsorcid{0000-0001-7598-5252}, E.~Gurpinar~Guler\cmsAuthorMark{70}\cmsorcid{0000-0002-6172-0285}, C.~Isik\cmsorcid{0000-0002-7977-0811}, O.~Kara, A.~Kayis~Topaksu\cmsorcid{0000-0002-3169-4573}, U.~Kiminsu\cmsorcid{0000-0001-6940-7800}, G.~Onengut\cmsorcid{0000-0002-6274-4254}, K.~Ozdemir\cmsAuthorMark{71}\cmsorcid{0000-0002-0103-1488}, A.~Polatoz\cmsorcid{0000-0001-9516-0821}, B.~Tali\cmsAuthorMark{72}\cmsorcid{0000-0002-7447-5602}, U.G.~Tok\cmsorcid{0000-0002-3039-021X}, S.~Turkcapar\cmsorcid{0000-0003-2608-0494}, E.~Uslan\cmsorcid{0000-0002-2472-0526}, I.S.~Zorbakir\cmsorcid{0000-0002-5962-2221}
\par}
\cmsinstitute{Middle East Technical University, Physics Department, Ankara, Turkey}
{\tolerance=6000
M.~Yalvac\cmsAuthorMark{73}\cmsorcid{0000-0003-4915-9162}
\par}
\cmsinstitute{Bogazici University, Istanbul, Turkey}
{\tolerance=6000
B.~Akgun\cmsorcid{0000-0001-8888-3562}, I.O.~Atakisi\cmsorcid{0000-0002-9231-7464}, E.~G\"{u}lmez\cmsorcid{0000-0002-6353-518X}, M.~Kaya\cmsAuthorMark{74}\cmsorcid{0000-0003-2890-4493}, O.~Kaya\cmsAuthorMark{75}\cmsorcid{0000-0002-8485-3822}, S.~Tekten\cmsAuthorMark{76}\cmsorcid{0000-0002-9624-5525}
\par}
\cmsinstitute{Istanbul Technical University, Istanbul, Turkey}
{\tolerance=6000
A.~Cakir\cmsorcid{0000-0002-8627-7689}, K.~Cankocak\cmsAuthorMark{69}$^{, }$\cmsAuthorMark{77}\cmsorcid{0000-0002-3829-3481}, Y.~Komurcu\cmsorcid{0000-0002-7084-030X}, S.~Sen\cmsAuthorMark{78}\cmsorcid{0000-0001-7325-1087}
\par}
\cmsinstitute{Istanbul University, Istanbul, Turkey}
{\tolerance=6000
O.~Aydilek\cmsorcid{0000-0002-2567-6766}, S.~Cerci\cmsAuthorMark{72}\cmsorcid{0000-0002-8702-6152}, V.~Epshteyn\cmsorcid{0000-0002-8863-6374}, B.~Hacisahinoglu\cmsorcid{0000-0002-2646-1230}, I.~Hos\cmsAuthorMark{79}\cmsorcid{0000-0002-7678-1101}, B.~Isildak\cmsAuthorMark{80}\cmsorcid{0000-0002-0283-5234}, B.~Kaynak\cmsorcid{0000-0003-3857-2496}, S.~Ozkorucuklu\cmsorcid{0000-0001-5153-9266}, O.~Potok\cmsorcid{0009-0005-1141-6401}, H.~Sert\cmsorcid{0000-0003-0716-6727}, C.~Simsek\cmsorcid{0000-0002-7359-8635}, D.~Sunar~Cerci\cmsAuthorMark{72}\cmsorcid{0000-0002-5412-4688}, C.~Zorbilmez\cmsorcid{0000-0002-5199-061X}
\par}
\cmsinstitute{Institute for Scintillation Materials of National Academy of Science of Ukraine, Kharkiv, Ukraine}
{\tolerance=6000
A.~Boyaryntsev\cmsorcid{0000-0001-9252-0430}, B.~Grynyov\cmsorcid{0000-0003-1700-0173}
\par}
\cmsinstitute{National Science Centre, Kharkiv Institute of Physics and Technology, Kharkiv, Ukraine}
{\tolerance=6000
L.~Levchuk\cmsorcid{0000-0001-5889-7410}
\par}
\cmsinstitute{University of Bristol, Bristol, United Kingdom}
{\tolerance=6000
D.~Anthony\cmsorcid{0000-0002-5016-8886}, J.J.~Brooke\cmsorcid{0000-0003-2529-0684}, A.~Bundock\cmsorcid{0000-0002-2916-6456}, F.~Bury\cmsorcid{0000-0002-3077-2090}, E.~Clement\cmsorcid{0000-0003-3412-4004}, D.~Cussans\cmsorcid{0000-0001-8192-0826}, H.~Flacher\cmsorcid{0000-0002-5371-941X}, M.~Glowacki, J.~Goldstein\cmsorcid{0000-0003-1591-6014}, H.F.~Heath\cmsorcid{0000-0001-6576-9740}, L.~Kreczko\cmsorcid{0000-0003-2341-8330}, B.~Krikler\cmsorcid{0000-0001-9712-0030}, S.~Paramesvaran\cmsorcid{0000-0003-4748-8296}, S.~Seif~El~Nasr-Storey, V.J.~Smith\cmsorcid{0000-0003-4543-2547}, N.~Stylianou\cmsAuthorMark{81}\cmsorcid{0000-0002-0113-6829}, K.~Walkingshaw~Pass, R.~White\cmsorcid{0000-0001-5793-526X}
\par}
\cmsinstitute{Rutherford Appleton Laboratory, Didcot, United Kingdom}
{\tolerance=6000
A.H.~Ball, K.W.~Bell\cmsorcid{0000-0002-2294-5860}, A.~Belyaev\cmsAuthorMark{82}\cmsorcid{0000-0002-1733-4408}, C.~Brew\cmsorcid{0000-0001-6595-8365}, R.M.~Brown\cmsorcid{0000-0002-6728-0153}, D.J.A.~Cockerill\cmsorcid{0000-0003-2427-5765}, C.~Cooke\cmsorcid{0000-0003-3730-4895}, K.V.~Ellis, K.~Harder\cmsorcid{0000-0002-2965-6973}, S.~Harper\cmsorcid{0000-0001-5637-2653}, M.-L.~Holmberg\cmsAuthorMark{83}\cmsorcid{0000-0002-9473-5985}, J.~Linacre\cmsorcid{0000-0001-7555-652X}, K.~Manolopoulos, D.M.~Newbold\cmsorcid{0000-0002-9015-9634}, E.~Olaiya, D.~Petyt\cmsorcid{0000-0002-2369-4469}, T.~Reis\cmsorcid{0000-0003-3703-6624}, G.~Salvi\cmsorcid{0000-0002-2787-1063}, T.~Schuh, C.H.~Shepherd-Themistocleous\cmsorcid{0000-0003-0551-6949}, I.R.~Tomalin\cmsorcid{0000-0003-2419-4439}, T.~Williams\cmsorcid{0000-0002-8724-4678}
\par}
\cmsinstitute{Imperial College, London, United Kingdom}
{\tolerance=6000
R.~Bainbridge\cmsorcid{0000-0001-9157-4832}, P.~Bloch\cmsorcid{0000-0001-6716-979X}, C.E.~Brown\cmsorcid{0000-0002-7766-6615}, O.~Buchmuller, V.~Cacchio, C.A.~Carrillo~Montoya\cmsorcid{0000-0002-6245-6535}, G.S.~Chahal\cmsAuthorMark{84}\cmsorcid{0000-0003-0320-4407}, D.~Colling\cmsorcid{0000-0001-9959-4977}, J.S.~Dancu, P.~Dauncey\cmsorcid{0000-0001-6839-9466}, G.~Davies\cmsorcid{0000-0001-8668-5001}, J.~Davies, M.~Della~Negra\cmsorcid{0000-0001-6497-8081}, S.~Fayer, G.~Fedi\cmsorcid{0000-0001-9101-2573}, G.~Hall\cmsorcid{0000-0002-6299-8385}, M.H.~Hassanshahi\cmsorcid{0000-0001-6634-4517}, A.~Howard, G.~Iles\cmsorcid{0000-0002-1219-5859}, M.~Knight\cmsorcid{0009-0008-1167-4816}, J.~Langford\cmsorcid{0000-0002-3931-4379}, L.~Lyons\cmsorcid{0000-0001-7945-9188}, A.-M.~Magnan\cmsorcid{0000-0002-4266-1646}, S.~Malik, A.~Martelli\cmsorcid{0000-0003-3530-2255}, M.~Mieskolainen\cmsorcid{0000-0001-8893-7401}, J.~Nash\cmsAuthorMark{85}\cmsorcid{0000-0003-0607-6519}, M.~Pesaresi, B.C.~Radburn-Smith\cmsorcid{0000-0003-1488-9675}, A.~Richards, A.~Rose\cmsorcid{0000-0002-9773-550X}, C.~Seez\cmsorcid{0000-0002-1637-5494}, R.~Shukla\cmsorcid{0000-0001-5670-5497}, A.~Tapper\cmsorcid{0000-0003-4543-864X}, K.~Uchida\cmsorcid{0000-0003-0742-2276}, G.P.~Uttley\cmsorcid{0009-0002-6248-6467}, L.H.~Vage, T.~Virdee\cmsAuthorMark{32}\cmsorcid{0000-0001-7429-2198}, M.~Vojinovic\cmsorcid{0000-0001-8665-2808}, N.~Wardle\cmsorcid{0000-0003-1344-3356}, D.~Winterbottom\cmsorcid{0000-0003-4582-150X}
\par}
\cmsinstitute{Brunel University, Uxbridge, United Kingdom}
{\tolerance=6000
K.~Coldham, J.E.~Cole\cmsorcid{0000-0001-5638-7599}, A.~Khan, P.~Kyberd\cmsorcid{0000-0002-7353-7090}, I.D.~Reid\cmsorcid{0000-0002-9235-779X}
\par}
\cmsinstitute{Baylor University, Waco, Texas, USA}
{\tolerance=6000
S.~Abdullin\cmsorcid{0000-0003-4885-6935}, A.~Brinkerhoff\cmsorcid{0000-0002-4819-7995}, B.~Caraway\cmsorcid{0000-0002-6088-2020}, J.~Dittmann\cmsorcid{0000-0002-1911-3158}, K.~Hatakeyama\cmsorcid{0000-0002-6012-2451}, J.~Hiltbrand\cmsorcid{0000-0003-1691-5937}, A.R.~Kanuganti\cmsorcid{0000-0002-0789-1200}, B.~McMaster\cmsorcid{0000-0002-4494-0446}, M.~Saunders\cmsorcid{0000-0003-1572-9075}, S.~Sawant\cmsorcid{0000-0002-1981-7753}, C.~Sutantawibul\cmsorcid{0000-0003-0600-0151}, M.~Toms\cmsAuthorMark{86}\cmsorcid{0000-0002-7703-3973}, J.~Wilson\cmsorcid{0000-0002-5672-7394}
\par}
\cmsinstitute{Catholic University of America, Washington, DC, USA}
{\tolerance=6000
R.~Bartek\cmsorcid{0000-0002-1686-2882}, A.~Dominguez\cmsorcid{0000-0002-7420-5493}, C.~Huerta~Escamilla, A.E.~Simsek\cmsorcid{0000-0002-9074-2256}, R.~Uniyal\cmsorcid{0000-0001-7345-6293}, A.M.~Vargas~Hernandez\cmsorcid{0000-0002-8911-7197}
\par}
\cmsinstitute{The University of Alabama, Tuscaloosa, Alabama, USA}
{\tolerance=6000
R.~Chudasama\cmsorcid{0009-0007-8848-6146}, S.I.~Cooper\cmsorcid{0000-0002-4618-0313}, S.V.~Gleyzer\cmsorcid{0000-0002-6222-8102}, C.U.~Perez\cmsorcid{0000-0002-6861-2674}, P.~Rumerio\cmsAuthorMark{87}\cmsorcid{0000-0002-1702-5541}, E.~Usai\cmsorcid{0000-0001-9323-2107}, C.~West\cmsorcid{0000-0003-4460-2241}, R.~Yi\cmsorcid{0000-0001-5818-1682}
\par}
\cmsinstitute{Boston University, Boston, Massachusetts, USA}
{\tolerance=6000
A.~Akpinar\cmsorcid{0000-0001-7510-6617}, A.~Albert\cmsorcid{0000-0003-2369-9507}, D.~Arcaro\cmsorcid{0000-0001-9457-8302}, C.~Cosby\cmsorcid{0000-0003-0352-6561}, Z.~Demiragli\cmsorcid{0000-0001-8521-737X}, C.~Erice\cmsorcid{0000-0002-6469-3200}, E.~Fontanesi\cmsorcid{0000-0002-0662-5904}, D.~Gastler\cmsorcid{0009-0000-7307-6311}, S.~Jeon\cmsorcid{0000-0003-1208-6940}, J.~Rohlf\cmsorcid{0000-0001-6423-9799}, K.~Salyer\cmsorcid{0000-0002-6957-1077}, D.~Sperka\cmsorcid{0000-0002-4624-2019}, D.~Spitzbart\cmsorcid{0000-0003-2025-2742}, I.~Suarez\cmsorcid{0000-0002-5374-6995}, A.~Tsatsos\cmsorcid{0000-0001-8310-8911}, S.~Yuan\cmsorcid{0000-0002-2029-024X}
\par}
\cmsinstitute{Brown University, Providence, Rhode Island, USA}
{\tolerance=6000
G.~Benelli\cmsorcid{0000-0003-4461-8905}, X.~Coubez\cmsAuthorMark{27}, D.~Cutts\cmsorcid{0000-0003-1041-7099}, M.~Hadley\cmsorcid{0000-0002-7068-4327}, U.~Heintz\cmsorcid{0000-0002-7590-3058}, J.M.~Hogan\cmsAuthorMark{88}\cmsorcid{0000-0002-8604-3452}, T.~Kwon\cmsorcid{0000-0001-9594-6277}, G.~Landsberg\cmsorcid{0000-0002-4184-9380}, K.T.~Lau\cmsorcid{0000-0003-1371-8575}, D.~Li\cmsorcid{0000-0003-0890-8948}, J.~Luo\cmsorcid{0000-0002-4108-8681}, S.~Mondal\cmsorcid{0000-0003-0153-7590}, M.~Narain$^{\textrm{\dag}}$\cmsorcid{0000-0002-7857-7403}, N.~Pervan\cmsorcid{0000-0002-8153-8464}, S.~Sagir\cmsAuthorMark{89}\cmsorcid{0000-0002-2614-5860}, F.~Simpson\cmsorcid{0000-0001-8944-9629}, M.~Stamenkovic\cmsorcid{0000-0003-2251-0610}, W.Y.~Wong, X.~Yan\cmsorcid{0000-0002-6426-0560}, W.~Zhang
\par}
\cmsinstitute{University of California, Davis, Davis, California, USA}
{\tolerance=6000
S.~Abbott\cmsorcid{0000-0002-7791-894X}, J.~Bonilla\cmsorcid{0000-0002-6982-6121}, C.~Brainerd\cmsorcid{0000-0002-9552-1006}, R.~Breedon\cmsorcid{0000-0001-5314-7581}, M.~Calderon~De~La~Barca~Sanchez\cmsorcid{0000-0001-9835-4349}, M.~Chertok\cmsorcid{0000-0002-2729-6273}, M.~Citron\cmsorcid{0000-0001-6250-8465}, J.~Conway\cmsorcid{0000-0003-2719-5779}, P.T.~Cox\cmsorcid{0000-0003-1218-2828}, R.~Erbacher\cmsorcid{0000-0001-7170-8944}, F.~Jensen\cmsorcid{0000-0003-3769-9081}, O.~Kukral\cmsorcid{0009-0007-3858-6659}, G.~Mocellin\cmsorcid{0000-0002-1531-3478}, M.~Mulhearn\cmsorcid{0000-0003-1145-6436}, D.~Pellett\cmsorcid{0009-0000-0389-8571}, W.~Wei\cmsorcid{0000-0003-4221-1802}, Y.~Yao\cmsorcid{0000-0002-5990-4245}, F.~Zhang\cmsorcid{0000-0002-6158-2468}
\par}
\cmsinstitute{University of California, Los Angeles, California, USA}
{\tolerance=6000
M.~Bachtis\cmsorcid{0000-0003-3110-0701}, R.~Cousins\cmsorcid{0000-0002-5963-0467}, A.~Datta\cmsorcid{0000-0003-2695-7719}, J.~Hauser\cmsorcid{0000-0002-9781-4873}, M.~Ignatenko\cmsorcid{0000-0001-8258-5863}, M.A.~Iqbal\cmsorcid{0000-0001-8664-1949}, T.~Lam\cmsorcid{0000-0002-0862-7348}, E.~Manca\cmsorcid{0000-0001-8946-655X}, D.~Saltzberg\cmsorcid{0000-0003-0658-9146}, V.~Valuev\cmsorcid{0000-0002-0783-6703}
\par}
\cmsinstitute{University of California, Riverside, Riverside, California, USA}
{\tolerance=6000
R.~Clare\cmsorcid{0000-0003-3293-5305}, J.W.~Gary\cmsorcid{0000-0003-0175-5731}, M.~Gordon, G.~Hanson\cmsorcid{0000-0002-7273-4009}, W.~Si\cmsorcid{0000-0002-5879-6326}, S.~Wimpenny$^{\textrm{\dag}}$\cmsorcid{0000-0003-0505-4908}
\par}
\cmsinstitute{University of California, San Diego, La Jolla, California, USA}
{\tolerance=6000
J.G.~Branson\cmsorcid{0009-0009-5683-4614}, S.~Cittolin\cmsorcid{0000-0002-0922-9587}, S.~Cooperstein\cmsorcid{0000-0003-0262-3132}, D.~Diaz\cmsorcid{0000-0001-6834-1176}, J.~Duarte\cmsorcid{0000-0002-5076-7096}, L.~Giannini\cmsorcid{0000-0002-5621-7706}, J.~Guiang\cmsorcid{0000-0002-2155-8260}, R.~Kansal\cmsorcid{0000-0003-2445-1060}, V.~Krutelyov\cmsorcid{0000-0002-1386-0232}, R.~Lee\cmsorcid{0009-0000-4634-0797}, J.~Letts\cmsorcid{0000-0002-0156-1251}, M.~Masciovecchio\cmsorcid{0000-0002-8200-9425}, F.~Mokhtar\cmsorcid{0000-0003-2533-3402}, M.~Pieri\cmsorcid{0000-0003-3303-6301}, M.~Quinnan\cmsorcid{0000-0003-2902-5597}, B.V.~Sathia~Narayanan\cmsorcid{0000-0003-2076-5126}, V.~Sharma\cmsorcid{0000-0003-1736-8795}, M.~Tadel\cmsorcid{0000-0001-8800-0045}, E.~Vourliotis\cmsorcid{0000-0002-2270-0492}, F.~W\"{u}rthwein\cmsorcid{0000-0001-5912-6124}, Y.~Xiang\cmsorcid{0000-0003-4112-7457}, A.~Yagil\cmsorcid{0000-0002-6108-4004}
\par}
\cmsinstitute{University of California, Santa Barbara - Department of Physics, Santa Barbara, California, USA}
{\tolerance=6000
A.~Barzdukas\cmsorcid{0000-0002-0518-3286}, L.~Brennan, C.~Campagnari\cmsorcid{0000-0002-8978-8177}, G.~Collura\cmsorcid{0000-0002-4160-1844}, A.~Dorsett\cmsorcid{0000-0001-5349-3011}, J.~Incandela\cmsorcid{0000-0001-9850-2030}, M.~Kilpatrick\cmsorcid{0000-0002-2602-0566}, J.~Kim\cmsorcid{0000-0002-2072-6082}, A.J.~Li\cmsorcid{0000-0002-3895-717X}, P.~Masterson\cmsorcid{0000-0002-6890-7624}, H.~Mei\cmsorcid{0000-0002-9838-8327}, M.~Oshiro\cmsorcid{0000-0002-2200-7516}, J.~Richman\cmsorcid{0000-0002-5189-146X}, U.~Sarica\cmsorcid{0000-0002-1557-4424}, R.~Schmitz\cmsorcid{0000-0003-2328-677X}, F.~Setti\cmsorcid{0000-0001-9800-7822}, J.~Sheplock\cmsorcid{0000-0002-8752-1946}, D.~Stuart\cmsorcid{0000-0002-4965-0747}, S.~Wang\cmsorcid{0000-0001-7887-1728}
\par}
\cmsinstitute{California Institute of Technology, Pasadena, California, USA}
{\tolerance=6000
A.~Bornheim\cmsorcid{0000-0002-0128-0871}, O.~Cerri, A.~Latorre, J.~Mao\cmsorcid{0009-0002-8988-9987}, H.B.~Newman\cmsorcid{0000-0003-0964-1480}, T.~Q.~Nguyen\cmsorcid{0000-0003-3954-5131}, M.~Spiropulu\cmsorcid{0000-0001-8172-7081}, J.R.~Vlimant\cmsorcid{0000-0002-9705-101X}, C.~Wang\cmsorcid{0000-0002-0117-7196}, S.~Xie\cmsorcid{0000-0003-2509-5731}, R.Y.~Zhu\cmsorcid{0000-0003-3091-7461}
\par}
\cmsinstitute{Carnegie Mellon University, Pittsburgh, Pennsylvania, USA}
{\tolerance=6000
J.~Alison\cmsorcid{0000-0003-0843-1641}, S.~An\cmsorcid{0000-0002-9740-1622}, M.B.~Andrews\cmsorcid{0000-0001-5537-4518}, P.~Bryant\cmsorcid{0000-0001-8145-6322}, V.~Dutta\cmsorcid{0000-0001-5958-829X}, T.~Ferguson\cmsorcid{0000-0001-5822-3731}, A.~Harilal\cmsorcid{0000-0001-9625-1987}, C.~Liu\cmsorcid{0000-0002-3100-7294}, T.~Mudholkar\cmsorcid{0000-0002-9352-8140}, S.~Murthy\cmsorcid{0000-0002-1277-9168}, M.~Paulini\cmsorcid{0000-0002-6714-5787}, A.~Roberts\cmsorcid{0000-0002-5139-0550}, A.~Sanchez\cmsorcid{0000-0002-5431-6989}, W.~Terrill\cmsorcid{0000-0002-2078-8419}
\par}
\cmsinstitute{University of Colorado Boulder, Boulder, Colorado, USA}
{\tolerance=6000
J.P.~Cumalat\cmsorcid{0000-0002-6032-5857}, W.T.~Ford\cmsorcid{0000-0001-8703-6943}, A.~Hassani\cmsorcid{0009-0008-4322-7682}, G.~Karathanasis\cmsorcid{0000-0001-5115-5828}, E.~MacDonald, N.~Manganelli\cmsorcid{0000-0002-3398-4531}, F.~Marini\cmsorcid{0000-0002-2374-6433}, A.~Perloff\cmsorcid{0000-0001-5230-0396}, C.~Savard\cmsorcid{0009-0000-7507-0570}, N.~Schonbeck\cmsorcid{0009-0008-3430-7269}, K.~Stenson\cmsorcid{0000-0003-4888-205X}, K.A.~Ulmer\cmsorcid{0000-0001-6875-9177}, S.R.~Wagner\cmsorcid{0000-0002-9269-5772}, N.~Zipper\cmsorcid{0000-0002-4805-8020}
\par}
\cmsinstitute{Cornell University, Ithaca, New York, USA}
{\tolerance=6000
J.~Alexander\cmsorcid{0000-0002-2046-342X}, S.~Bright-Thonney\cmsorcid{0000-0003-1889-7824}, X.~Chen\cmsorcid{0000-0002-8157-1328}, D.J.~Cranshaw\cmsorcid{0000-0002-7498-2129}, J.~Fan\cmsorcid{0009-0003-3728-9960}, X.~Fan\cmsorcid{0000-0003-2067-0127}, D.~Gadkari\cmsorcid{0000-0002-6625-8085}, S.~Hogan\cmsorcid{0000-0003-3657-2281}, J.~Monroy\cmsorcid{0000-0002-7394-4710}, J.R.~Patterson\cmsorcid{0000-0002-3815-3649}, J.~Reichert\cmsorcid{0000-0003-2110-8021}, M.~Reid\cmsorcid{0000-0001-7706-1416}, A.~Ryd\cmsorcid{0000-0001-5849-1912}, J.~Thom\cmsorcid{0000-0002-4870-8468}, P.~Wittich\cmsorcid{0000-0002-7401-2181}, R.~Zou\cmsorcid{0000-0002-0542-1264}
\par}
\cmsinstitute{Fermi National Accelerator Laboratory, Batavia, Illinois, USA}
{\tolerance=6000
M.~Albrow\cmsorcid{0000-0001-7329-4925}, M.~Alyari\cmsorcid{0000-0001-9268-3360}, O.~Amram\cmsorcid{0000-0002-3765-3123}, G.~Apollinari\cmsorcid{0000-0002-5212-5396}, A.~Apresyan\cmsorcid{0000-0002-6186-0130}, L.A.T.~Bauerdick\cmsorcid{0000-0002-7170-9012}, D.~Berry\cmsorcid{0000-0002-5383-8320}, J.~Berryhill\cmsorcid{0000-0002-8124-3033}, P.C.~Bhat\cmsorcid{0000-0003-3370-9246}, K.~Burkett\cmsorcid{0000-0002-2284-4744}, J.N.~Butler\cmsorcid{0000-0002-0745-8618}, A.~Canepa\cmsorcid{0000-0003-4045-3998}, G.B.~Cerati\cmsorcid{0000-0003-3548-0262}, H.W.K.~Cheung\cmsorcid{0000-0001-6389-9357}, F.~Chlebana\cmsorcid{0000-0002-8762-8559}, G.~Cummings\cmsorcid{0000-0002-8045-7806}, J.~Dickinson\cmsorcid{0000-0001-5450-5328}, I.~Dutta\cmsorcid{0000-0003-0953-4503}, V.D.~Elvira\cmsorcid{0000-0003-4446-4395}, Y.~Feng\cmsorcid{0000-0003-2812-338X}, J.~Freeman\cmsorcid{0000-0002-3415-5671}, A.~Gandrakota\cmsorcid{0000-0003-4860-3233}, Z.~Gecse\cmsorcid{0009-0009-6561-3418}, L.~Gray\cmsorcid{0000-0002-6408-4288}, D.~Green, A.~Grummer\cmsorcid{0000-0003-2752-1183}, S.~Gr\"{u}nendahl\cmsorcid{0000-0002-4857-0294}, D.~Guerrero\cmsorcid{0000-0001-5552-5400}, O.~Gutsche\cmsorcid{0000-0002-8015-9622}, R.M.~Harris\cmsorcid{0000-0003-1461-3425}, R.~Heller\cmsorcid{0000-0002-7368-6723}, T.C.~Herwig\cmsorcid{0000-0002-4280-6382}, J.~Hirschauer\cmsorcid{0000-0002-8244-0805}, L.~Horyn\cmsorcid{0000-0002-9512-4932}, B.~Jayatilaka\cmsorcid{0000-0001-7912-5612}, S.~Jindariani\cmsorcid{0009-0000-7046-6533}, M.~Johnson\cmsorcid{0000-0001-7757-8458}, U.~Joshi\cmsorcid{0000-0001-8375-0760}, T.~Klijnsma\cmsorcid{0000-0003-1675-6040}, B.~Klima\cmsorcid{0000-0002-3691-7625}, K.H.M.~Kwok\cmsorcid{0000-0002-8693-6146}, S.~Lammel\cmsorcid{0000-0003-0027-635X}, D.~Lincoln\cmsorcid{0000-0002-0599-7407}, R.~Lipton\cmsorcid{0000-0002-6665-7289}, T.~Liu\cmsorcid{0009-0007-6522-5605}, C.~Madrid\cmsorcid{0000-0003-3301-2246}, K.~Maeshima\cmsorcid{0009-0000-2822-897X}, C.~Mantilla\cmsorcid{0000-0002-0177-5903}, D.~Mason\cmsorcid{0000-0002-0074-5390}, P.~McBride\cmsorcid{0000-0001-6159-7750}, P.~Merkel\cmsorcid{0000-0003-4727-5442}, S.~Mrenna\cmsorcid{0000-0001-8731-160X}, S.~Nahn\cmsorcid{0000-0002-8949-0178}, J.~Ngadiuba\cmsorcid{0000-0002-0055-2935}, D.~Noonan\cmsorcid{0000-0002-3932-3769}, V.~Papadimitriou\cmsorcid{0000-0002-0690-7186}, N.~Pastika\cmsorcid{0009-0006-0993-6245}, K.~Pedro\cmsorcid{0000-0003-2260-9151}, C.~Pena\cmsAuthorMark{90}\cmsorcid{0000-0002-4500-7930}, F.~Ravera\cmsorcid{0000-0003-3632-0287}, A.~Reinsvold~Hall\cmsAuthorMark{91}\cmsorcid{0000-0003-1653-8553}, L.~Ristori\cmsorcid{0000-0003-1950-2492}, E.~Sexton-Kennedy\cmsorcid{0000-0001-9171-1980}, N.~Smith\cmsorcid{0000-0002-0324-3054}, A.~Soha\cmsorcid{0000-0002-5968-1192}, L.~Spiegel\cmsorcid{0000-0001-9672-1328}, S.~Stoynev\cmsorcid{0000-0003-4563-7702}, J.~Strait\cmsorcid{0000-0002-7233-8348}, L.~Taylor\cmsorcid{0000-0002-6584-2538}, S.~Tkaczyk\cmsorcid{0000-0001-7642-5185}, N.V.~Tran\cmsorcid{0000-0002-8440-6854}, L.~Uplegger\cmsorcid{0000-0002-9202-803X}, E.W.~Vaandering\cmsorcid{0000-0003-3207-6950}, I.~Zoi\cmsorcid{0000-0002-5738-9446}
\par}
\cmsinstitute{University of Florida, Gainesville, Florida, USA}
{\tolerance=6000
C.~Aruta\cmsorcid{0000-0001-9524-3264}, P.~Avery\cmsorcid{0000-0003-0609-627X}, D.~Bourilkov\cmsorcid{0000-0003-0260-4935}, L.~Cadamuro\cmsorcid{0000-0001-8789-610X}, P.~Chang\cmsorcid{0000-0002-2095-6320}, V.~Cherepanov\cmsorcid{0000-0002-6748-4850}, R.D.~Field, E.~Koenig\cmsorcid{0000-0002-0884-7922}, M.~Kolosova\cmsorcid{0000-0002-5838-2158}, J.~Konigsberg\cmsorcid{0000-0001-6850-8765}, A.~Korytov\cmsorcid{0000-0001-9239-3398}, K.H.~Lo, K.~Matchev\cmsorcid{0000-0003-4182-9096}, N.~Menendez\cmsorcid{0000-0002-3295-3194}, G.~Mitselmakher\cmsorcid{0000-0001-5745-3658}, K.~Mohrman\cmsorcid{0009-0007-2940-0496}, A.~Muthirakalayil~Madhu\cmsorcid{0000-0003-1209-3032}, N.~Rawal\cmsorcid{0000-0002-7734-3170}, D.~Rosenzweig\cmsorcid{0000-0002-3687-5189}, S.~Rosenzweig\cmsorcid{0000-0002-5613-1507}, K.~Shi\cmsorcid{0000-0002-2475-0055}, J.~Wang\cmsorcid{0000-0003-3879-4873}
\par}
\cmsinstitute{Florida State University, Tallahassee, Florida, USA}
{\tolerance=6000
T.~Adams\cmsorcid{0000-0001-8049-5143}, A.~Al~Kadhim\cmsorcid{0000-0003-3490-8407}, A.~Askew\cmsorcid{0000-0002-7172-1396}, N.~Bower\cmsorcid{0000-0001-8775-0696}, R.~Habibullah\cmsorcid{0000-0002-3161-8300}, V.~Hagopian\cmsorcid{0000-0002-3791-1989}, R.~Hashmi\cmsorcid{0000-0002-5439-8224}, R.S.~Kim\cmsorcid{0000-0002-8645-186X}, S.~Kim\cmsorcid{0000-0003-2381-5117}, T.~Kolberg\cmsorcid{0000-0002-0211-6109}, G.~Martinez, H.~Prosper\cmsorcid{0000-0002-4077-2713}, P.R.~Prova, O.~Viazlo\cmsorcid{0000-0002-2957-0301}, M.~Wulansatiti\cmsorcid{0000-0001-6794-3079}, R.~Yohay\cmsorcid{0000-0002-0124-9065}, J.~Zhang
\par}
\cmsinstitute{Florida Institute of Technology, Melbourne, Florida, USA}
{\tolerance=6000
B.~Alsufyani, M.M.~Baarmand\cmsorcid{0000-0002-9792-8619}, S.~Butalla\cmsorcid{0000-0003-3423-9581}, T.~Elkafrawy\cmsAuthorMark{56}\cmsorcid{0000-0001-9930-6445}, M.~Hohlmann\cmsorcid{0000-0003-4578-9319}, R.~Kumar~Verma\cmsorcid{0000-0002-8264-156X}, M.~Rahmani
\par}
\cmsinstitute{University of Illinois at Chicago (UIC), Chicago, Illinois, USA}
{\tolerance=6000
M.R.~Adams\cmsorcid{0000-0001-8493-3737}, C.~Bennett, R.~Cavanaugh\cmsorcid{0000-0001-7169-3420}, S.~Dittmer\cmsorcid{0000-0002-5359-9614}, R.~Escobar~Franco\cmsorcid{0000-0003-2090-5010}, O.~Evdokimov\cmsorcid{0000-0002-1250-8931}, C.E.~Gerber\cmsorcid{0000-0002-8116-9021}, D.J.~Hofman\cmsorcid{0000-0002-2449-3845}, J.h.~Lee\cmsorcid{0000-0002-5574-4192}, D.~S.~Lemos\cmsorcid{0000-0003-1982-8978}, A.H.~Merrit\cmsorcid{0000-0003-3922-6464}, C.~Mills\cmsorcid{0000-0001-8035-4818}, S.~Nanda\cmsorcid{0000-0003-0550-4083}, G.~Oh\cmsorcid{0000-0003-0744-1063}, B.~Ozek\cmsorcid{0009-0000-2570-1100}, D.~Pilipovic\cmsorcid{0000-0002-4210-2780}, T.~Roy\cmsorcid{0000-0001-7299-7653}, S.~Rudrabhatla\cmsorcid{0000-0002-7366-4225}, M.B.~Tonjes\cmsorcid{0000-0002-2617-9315}, N.~Varelas\cmsorcid{0000-0002-9397-5514}, X.~Wang\cmsorcid{0000-0003-2792-8493}, Z.~Ye\cmsorcid{0000-0001-6091-6772}, J.~Yoo\cmsorcid{0000-0002-3826-1332}
\par}
\cmsinstitute{The University of Iowa, Iowa City, Iowa, USA}
{\tolerance=6000
M.~Alhusseini\cmsorcid{0000-0002-9239-470X}, D.~Blend, K.~Dilsiz\cmsAuthorMark{92}\cmsorcid{0000-0003-0138-3368}, L.~Emediato\cmsorcid{0000-0002-3021-5032}, G.~Karaman\cmsorcid{0000-0001-8739-9648}, O.K.~K\"{o}seyan\cmsorcid{0000-0001-9040-3468}, J.-P.~Merlo, A.~Mestvirishvili\cmsAuthorMark{93}\cmsorcid{0000-0002-8591-5247}, J.~Nachtman\cmsorcid{0000-0003-3951-3420}, O.~Neogi, H.~Ogul\cmsAuthorMark{94}\cmsorcid{0000-0002-5121-2893}, Y.~Onel\cmsorcid{0000-0002-8141-7769}, A.~Penzo\cmsorcid{0000-0003-3436-047X}, C.~Snyder, E.~Tiras\cmsAuthorMark{95}\cmsorcid{0000-0002-5628-7464}
\par}
\cmsinstitute{Johns Hopkins University, Baltimore, Maryland, USA}
{\tolerance=6000
B.~Blumenfeld\cmsorcid{0000-0003-1150-1735}, L.~Corcodilos\cmsorcid{0000-0001-6751-3108}, J.~Davis\cmsorcid{0000-0001-6488-6195}, A.V.~Gritsan\cmsorcid{0000-0002-3545-7970}, L.~Kang\cmsorcid{0000-0002-0941-4512}, S.~Kyriacou\cmsorcid{0000-0002-9254-4368}, P.~Maksimovic\cmsorcid{0000-0002-2358-2168}, M.~Roguljic\cmsorcid{0000-0001-5311-3007}, J.~Roskes\cmsorcid{0000-0001-8761-0490}, S.~Sekhar\cmsorcid{0000-0002-8307-7518}, M.~Swartz\cmsorcid{0000-0002-0286-5070}, T.\'{A}.~V\'{a}mi\cmsorcid{0000-0002-0959-9211}
\par}
\cmsinstitute{The University of Kansas, Lawrence, Kansas, USA}
{\tolerance=6000
A.~Abreu\cmsorcid{0000-0002-9000-2215}, L.F.~Alcerro~Alcerro\cmsorcid{0000-0001-5770-5077}, J.~Anguiano\cmsorcid{0000-0002-7349-350X}, P.~Baringer\cmsorcid{0000-0002-3691-8388}, A.~Bean\cmsorcid{0000-0001-5967-8674}, Z.~Flowers\cmsorcid{0000-0001-8314-2052}, D.~Grove, J.~King\cmsorcid{0000-0001-9652-9854}, G.~Krintiras\cmsorcid{0000-0002-0380-7577}, M.~Lazarovits\cmsorcid{0000-0002-5565-3119}, C.~Le~Mahieu\cmsorcid{0000-0001-5924-1130}, C.~Lindsey, J.~Marquez\cmsorcid{0000-0003-3887-4048}, N.~Minafra\cmsorcid{0000-0003-4002-1888}, M.~Murray\cmsorcid{0000-0001-7219-4818}, M.~Nickel\cmsorcid{0000-0003-0419-1329}, M.~Pitt\cmsorcid{0000-0003-2461-5985}, S.~Popescu\cmsAuthorMark{96}\cmsorcid{0000-0002-0345-2171}, C.~Rogan\cmsorcid{0000-0002-4166-4503}, C.~Royon\cmsorcid{0000-0002-7672-9709}, R.~Salvatico\cmsorcid{0000-0002-2751-0567}, S.~Sanders\cmsorcid{0000-0002-9491-6022}, C.~Smith\cmsorcid{0000-0003-0505-0528}, Q.~Wang\cmsorcid{0000-0003-3804-3244}, G.~Wilson\cmsorcid{0000-0003-0917-4763}
\par}
\cmsinstitute{Kansas State University, Manhattan, Kansas, USA}
{\tolerance=6000
B.~Allmond\cmsorcid{0000-0002-5593-7736}, A.~Ivanov\cmsorcid{0000-0002-9270-5643}, K.~Kaadze\cmsorcid{0000-0003-0571-163X}, A.~Kalogeropoulos\cmsorcid{0000-0003-3444-0314}, D.~Kim, Y.~Maravin\cmsorcid{0000-0002-9449-0666}, K.~Nam, J.~Natoli\cmsorcid{0000-0001-6675-3564}, D.~Roy\cmsorcid{0000-0002-8659-7762}, G.~Sorrentino\cmsorcid{0000-0002-2253-819X}
\par}
\cmsinstitute{Lawrence Livermore National Laboratory, Livermore, California, USA}
{\tolerance=6000
F.~Rebassoo\cmsorcid{0000-0001-8934-9329}, D.~Wright\cmsorcid{0000-0002-3586-3354}
\par}
\cmsinstitute{University of Maryland, College Park, Maryland, USA}
{\tolerance=6000
A.~Baden\cmsorcid{0000-0002-6159-3861}, A.~Belloni\cmsorcid{0000-0002-1727-656X}, A.~Bethani\cmsorcid{0000-0002-8150-7043}, Y.M.~Chen\cmsorcid{0000-0002-5795-4783}, S.C.~Eno\cmsorcid{0000-0003-4282-2515}, N.J.~Hadley\cmsorcid{0000-0002-1209-6471}, S.~Jabeen\cmsorcid{0000-0002-0155-7383}, R.G.~Kellogg\cmsorcid{0000-0001-9235-521X}, T.~Koeth\cmsorcid{0000-0002-0082-0514}, Y.~Lai\cmsorcid{0000-0002-7795-8693}, S.~Lascio\cmsorcid{0000-0001-8579-5874}, A.C.~Mignerey\cmsorcid{0000-0001-5164-6969}, S.~Nabili\cmsorcid{0000-0002-6893-1018}, C.~Palmer\cmsorcid{0000-0002-5801-5737}, C.~Papageorgakis\cmsorcid{0000-0003-4548-0346}, M.M.~Paranjpe, L.~Wang\cmsorcid{0000-0003-3443-0626}
\par}
\cmsinstitute{Massachusetts Institute of Technology, Cambridge, Massachusetts, USA}
{\tolerance=6000
J.~Bendavid\cmsorcid{0000-0002-7907-1789}, W.~Busza\cmsorcid{0000-0002-3831-9071}, I.A.~Cali\cmsorcid{0000-0002-2822-3375}, Y.~Chen\cmsorcid{0000-0003-2582-6469}, M.~D'Alfonso\cmsorcid{0000-0002-7409-7904}, J.~Eysermans\cmsorcid{0000-0001-6483-7123}, C.~Freer\cmsorcid{0000-0002-7967-4635}, G.~Gomez-Ceballos\cmsorcid{0000-0003-1683-9460}, M.~Goncharov, P.~Harris, D.~Hoang, D.~Kovalskyi\cmsorcid{0000-0002-6923-293X}, J.~Krupa\cmsorcid{0000-0003-0785-7552}, L.~Lavezzo\cmsorcid{0000-0002-1364-9920}, Y.-J.~Lee\cmsorcid{0000-0003-2593-7767}, K.~Long\cmsorcid{0000-0003-0664-1653}, C.~Mironov\cmsorcid{0000-0002-8599-2437}, C.~Paus\cmsorcid{0000-0002-6047-4211}, D.~Rankin\cmsorcid{0000-0001-8411-9620}, C.~Roland\cmsorcid{0000-0002-7312-5854}, G.~Roland\cmsorcid{0000-0001-8983-2169}, S.~Rothman\cmsorcid{0000-0002-1377-9119}, Z.~Shi\cmsorcid{0000-0001-5498-8825}, G.S.F.~Stephans\cmsorcid{0000-0003-3106-4894}, J.~Wang, Z.~Wang\cmsorcid{0000-0002-3074-3767}, B.~Wyslouch\cmsorcid{0000-0003-3681-0649}, T.~J.~Yang\cmsorcid{0000-0003-4317-4660}
\par}
\cmsinstitute{University of Minnesota, Minneapolis, Minnesota, USA}
{\tolerance=6000
B.~Crossman\cmsorcid{0000-0002-2700-5085}, B.M.~Joshi\cmsorcid{0000-0002-4723-0968}, C.~Kapsiak\cmsorcid{0009-0008-7743-5316}, M.~Krohn\cmsorcid{0000-0002-1711-2506}, D.~Mahon\cmsorcid{0000-0002-2640-5941}, J.~Mans\cmsorcid{0000-0003-2840-1087}, B.~Marzocchi\cmsorcid{0000-0001-6687-6214}, S.~Pandey\cmsorcid{0000-0003-0440-6019}, M.~Revering\cmsorcid{0000-0001-5051-0293}, R.~Rusack\cmsorcid{0000-0002-7633-749X}, R.~Saradhy\cmsorcid{0000-0001-8720-293X}, N.~Schroeder\cmsorcid{0000-0002-8336-6141}, N.~Strobbe\cmsorcid{0000-0001-8835-8282}, M.A.~Wadud\cmsorcid{0000-0002-0653-0761}
\par}
\cmsinstitute{University of Mississippi, Oxford, Mississippi, USA}
{\tolerance=6000
L.M.~Cremaldi\cmsorcid{0000-0001-5550-7827}
\par}
\cmsinstitute{University of Nebraska-Lincoln, Lincoln, Nebraska, USA}
{\tolerance=6000
K.~Bloom\cmsorcid{0000-0002-4272-8900}, M.~Bryson, D.R.~Claes\cmsorcid{0000-0003-4198-8919}, C.~Fangmeier\cmsorcid{0000-0002-5998-8047}, F.~Golf\cmsorcid{0000-0003-3567-9351}, G.~Haza\cmsorcid{0009-0001-1326-3956}, J.~Hossain\cmsorcid{0000-0001-5144-7919}, C.~Joo\cmsorcid{0000-0002-5661-4330}, I.~Kravchenko\cmsorcid{0000-0003-0068-0395}, I.~Reed\cmsorcid{0000-0002-1823-8856}, J.E.~Siado\cmsorcid{0000-0002-9757-470X}, W.~Tabb\cmsorcid{0000-0002-9542-4847}, A.~Vagnerini\cmsorcid{0000-0001-8730-5031}, A.~Wightman\cmsorcid{0000-0001-6651-5320}, F.~Yan\cmsorcid{0000-0002-4042-0785}, D.~Yu\cmsorcid{0000-0001-5921-5231}, A.G.~Zecchinelli\cmsorcid{0000-0001-8986-278X}
\par}
\cmsinstitute{State University of New York at Buffalo, Buffalo, New York, USA}
{\tolerance=6000
G.~Agarwal\cmsorcid{0000-0002-2593-5297}, H.~Bandyopadhyay\cmsorcid{0000-0001-9726-4915}, L.~Hay\cmsorcid{0000-0002-7086-7641}, I.~Iashvili\cmsorcid{0000-0003-1948-5901}, A.~Kharchilava\cmsorcid{0000-0002-3913-0326}, M.~Morris\cmsorcid{0000-0002-2830-6488}, D.~Nguyen\cmsorcid{0000-0002-5185-8504}, S.~Rappoccio\cmsorcid{0000-0002-5449-2560}, H.~Rejeb~Sfar, A.~Williams\cmsorcid{0000-0003-4055-6532}
\par}
\cmsinstitute{Northeastern University, Boston, Massachusetts, USA}
{\tolerance=6000
E.~Barberis\cmsorcid{0000-0002-6417-5913}, Y.~Haddad\cmsorcid{0000-0003-4916-7752}, Y.~Han\cmsorcid{0000-0002-3510-6505}, A.~Krishna\cmsorcid{0000-0002-4319-818X}, J.~Li\cmsorcid{0000-0001-5245-2074}, M.~Lu\cmsorcid{0000-0002-6999-3931}, G.~Madigan\cmsorcid{0000-0001-8796-5865}, R.~Mccarthy\cmsorcid{0000-0002-9391-2599}, D.M.~Morse\cmsorcid{0000-0003-3163-2169}, V.~Nguyen\cmsorcid{0000-0003-1278-9208}, T.~Orimoto\cmsorcid{0000-0002-8388-3341}, A.~Parker\cmsorcid{0000-0002-9421-3335}, L.~Skinnari\cmsorcid{0000-0002-2019-6755}, A.~Tishelman-Charny\cmsorcid{0000-0002-7332-5098}, B.~Wang\cmsorcid{0000-0003-0796-2475}, D.~Wood\cmsorcid{0000-0002-6477-801X}
\par}
\cmsinstitute{Northwestern University, Evanston, Illinois, USA}
{\tolerance=6000
S.~Bhattacharya\cmsorcid{0000-0002-0526-6161}, J.~Bueghly, Z.~Chen\cmsorcid{0000-0003-4521-6086}, K.A.~Hahn\cmsorcid{0000-0001-7892-1676}, Y.~Liu\cmsorcid{0000-0002-5588-1760}, Y.~Miao\cmsorcid{0000-0002-2023-2082}, D.G.~Monk\cmsorcid{0000-0002-8377-1999}, M.H.~Schmitt\cmsorcid{0000-0003-0814-3578}, A.~Taliercio\cmsorcid{0000-0002-5119-6280}, M.~Velasco
\par}
\cmsinstitute{University of Notre Dame, Notre Dame, Indiana, USA}
{\tolerance=6000
R.~Band\cmsorcid{0000-0003-4873-0523}, R.~Bucci, S.~Castells\cmsorcid{0000-0003-2618-3856}, M.~Cremonesi, A.~Das\cmsorcid{0000-0001-9115-9698}, R.~Goldouzian\cmsorcid{0000-0002-0295-249X}, M.~Hildreth\cmsorcid{0000-0002-4454-3934}, K.W.~Ho\cmsorcid{0000-0003-2229-7223}, K.~Hurtado~Anampa\cmsorcid{0000-0002-9779-3566}, T.~Ivanov\cmsorcid{0000-0003-0489-9191}, C.~Jessop\cmsorcid{0000-0002-6885-3611}, K.~Lannon\cmsorcid{0000-0002-9706-0098}, J.~Lawrence\cmsorcid{0000-0001-6326-7210}, N.~Loukas\cmsorcid{0000-0003-0049-6918}, L.~Lutton\cmsorcid{0000-0002-3212-4505}, J.~Mariano, N.~Marinelli, I.~Mcalister, T.~McCauley\cmsorcid{0000-0001-6589-8286}, C.~Mcgrady\cmsorcid{0000-0002-8821-2045}, C.~Moore\cmsorcid{0000-0002-8140-4183}, Y.~Musienko\cmsAuthorMark{16}\cmsorcid{0009-0006-3545-1938}, H.~Nelson\cmsorcid{0000-0001-5592-0785}, M.~Osherson\cmsorcid{0000-0002-9760-9976}, A.~Piccinelli\cmsorcid{0000-0003-0386-0527}, R.~Ruchti\cmsorcid{0000-0002-3151-1386}, A.~Townsend\cmsorcid{0000-0002-3696-689X}, Y.~Wan, M.~Wayne\cmsorcid{0000-0001-8204-6157}, H.~Yockey, M.~Zarucki\cmsorcid{0000-0003-1510-5772}, L.~Zygala\cmsorcid{0000-0001-9665-7282}
\par}
\cmsinstitute{The Ohio State University, Columbus, Ohio, USA}
{\tolerance=6000
A.~Basnet\cmsorcid{0000-0001-8460-0019}, B.~Bylsma, M.~Carrigan\cmsorcid{0000-0003-0538-5854}, L.S.~Durkin\cmsorcid{0000-0002-0477-1051}, C.~Hill\cmsorcid{0000-0003-0059-0779}, M.~Joyce\cmsorcid{0000-0003-1112-5880}, A.~Lesauvage\cmsorcid{0000-0003-3437-7845}, M.~Nunez~Ornelas\cmsorcid{0000-0003-2663-7379}, K.~Wei, B.L.~Winer\cmsorcid{0000-0001-9980-4698}, B.~R.~Yates\cmsorcid{0000-0001-7366-1318}
\par}
\cmsinstitute{Princeton University, Princeton, New Jersey, USA}
{\tolerance=6000
F.M.~Addesa\cmsorcid{0000-0003-0484-5804}, H.~Bouchamaoui\cmsorcid{0000-0002-9776-1935}, P.~Das\cmsorcid{0000-0002-9770-1377}, G.~Dezoort\cmsorcid{0000-0002-5890-0445}, P.~Elmer\cmsorcid{0000-0001-6830-3356}, A.~Frankenthal\cmsorcid{0000-0002-2583-5982}, B.~Greenberg\cmsorcid{0000-0002-4922-1934}, N.~Haubrich\cmsorcid{0000-0002-7625-8169}, S.~Higginbotham\cmsorcid{0000-0002-4436-5461}, G.~Kopp\cmsorcid{0000-0001-8160-0208}, S.~Kwan\cmsorcid{0000-0002-5308-7707}, D.~Lange\cmsorcid{0000-0002-9086-5184}, A.~Loeliger\cmsorcid{0000-0002-5017-1487}, D.~Marlow\cmsorcid{0000-0002-6395-1079}, I.~Ojalvo\cmsorcid{0000-0003-1455-6272}, J.~Olsen\cmsorcid{0000-0002-9361-5762}, A.~Shevelev\cmsorcid{0000-0003-4600-0228}, D.~Stickland\cmsorcid{0000-0003-4702-8820}, C.~Tully\cmsorcid{0000-0001-6771-2174}
\par}
\cmsinstitute{University of Puerto Rico, Mayaguez, Puerto Rico, USA}
{\tolerance=6000
S.~Malik\cmsorcid{0000-0002-6356-2655}
\par}
\cmsinstitute{Purdue University, West Lafayette, Indiana, USA}
{\tolerance=6000
A.S.~Bakshi\cmsorcid{0000-0002-2857-6883}, V.E.~Barnes\cmsorcid{0000-0001-6939-3445}, S.~Chandra\cmsorcid{0009-0000-7412-4071}, R.~Chawla\cmsorcid{0000-0003-4802-6819}, S.~Das\cmsorcid{0000-0001-6701-9265}, A.~Gu\cmsorcid{0000-0002-6230-1138}, L.~Gutay, M.~Jones\cmsorcid{0000-0002-9951-4583}, A.W.~Jung\cmsorcid{0000-0003-3068-3212}, D.~Kondratyev\cmsorcid{0000-0002-7874-2480}, A.M.~Koshy, M.~Liu\cmsorcid{0000-0001-9012-395X}, G.~Negro\cmsorcid{0000-0002-1418-2154}, N.~Neumeister\cmsorcid{0000-0003-2356-1700}, G.~Paspalaki\cmsorcid{0000-0001-6815-1065}, S.~Piperov\cmsorcid{0000-0002-9266-7819}, V.~Scheurer, J.F.~Schulte\cmsorcid{0000-0003-4421-680X}, M.~Stojanovic\cmsorcid{0000-0002-1542-0855}, J.~Thieman\cmsorcid{0000-0001-7684-6588}, A.~K.~Virdi\cmsorcid{0000-0002-0866-8932}, F.~Wang\cmsorcid{0000-0002-8313-0809}, W.~Xie\cmsorcid{0000-0003-1430-9191}
\par}
\cmsinstitute{Purdue University Northwest, Hammond, Indiana, USA}
{\tolerance=6000
J.~Dolen\cmsorcid{0000-0003-1141-3823}, N.~Parashar\cmsorcid{0009-0009-1717-0413}, A.~Pathak\cmsorcid{0000-0001-9861-2942}
\par}
\cmsinstitute{Rice University, Houston, Texas, USA}
{\tolerance=6000
D.~Acosta\cmsorcid{0000-0001-5367-1738}, A.~Baty\cmsorcid{0000-0001-5310-3466}, T.~Carnahan\cmsorcid{0000-0001-7492-3201}, K.M.~Ecklund\cmsorcid{0000-0002-6976-4637}, P.J.~Fern\'{a}ndez~Manteca\cmsorcid{0000-0003-2566-7496}, S.~Freed, P.~Gardner, F.J.M.~Geurts\cmsorcid{0000-0003-2856-9090}, A.~Kumar\cmsorcid{0000-0002-5180-6595}, W.~Li\cmsorcid{0000-0003-4136-3409}, O.~Miguel~Colin\cmsorcid{0000-0001-6612-432X}, B.P.~Padley\cmsorcid{0000-0002-3572-5701}, R.~Redjimi, J.~Rotter\cmsorcid{0009-0009-4040-7407}, E.~Yigitbasi\cmsorcid{0000-0002-9595-2623}, Y.~Zhang\cmsorcid{0000-0002-6812-761X}
\par}
\cmsinstitute{University of Rochester, Rochester, New York, USA}
{\tolerance=6000
A.~Bodek\cmsorcid{0000-0003-0409-0341}, P.~de~Barbaro\cmsorcid{0000-0002-5508-1827}, R.~Demina\cmsorcid{0000-0002-7852-167X}, J.L.~Dulemba\cmsorcid{0000-0002-9842-7015}, C.~Fallon, A.~Garcia-Bellido\cmsorcid{0000-0002-1407-1972}, O.~Hindrichs\cmsorcid{0000-0001-7640-5264}, A.~Khukhunaishvili\cmsorcid{0000-0002-3834-1316}, P.~Parygin\cmsAuthorMark{86}\cmsorcid{0000-0001-6743-3781}, E.~Popova\cmsAuthorMark{86}\cmsorcid{0000-0001-7556-8969}, R.~Taus\cmsorcid{0000-0002-5168-2932}, G.P.~Van~Onsem\cmsorcid{0000-0002-1664-2337}
\par}
\cmsinstitute{The Rockefeller University, New York, New York, USA}
{\tolerance=6000
K.~Goulianos\cmsorcid{0000-0002-6230-9535}
\par}
\cmsinstitute{Rutgers, The State University of New Jersey, Piscataway, New Jersey, USA}
{\tolerance=6000
B.~Chiarito, J.P.~Chou\cmsorcid{0000-0001-6315-905X}, Y.~Gershtein\cmsorcid{0000-0002-4871-5449}, E.~Halkiadakis\cmsorcid{0000-0002-3584-7856}, A.~Hart\cmsorcid{0000-0003-2349-6582}, M.~Heindl\cmsorcid{0000-0002-2831-463X}, D.~Jaroslawski\cmsorcid{0000-0003-2497-1242}, O.~Karacheban\cmsAuthorMark{30}\cmsorcid{0000-0002-2785-3762}, I.~Laflotte\cmsorcid{0000-0002-7366-8090}, A.~Lath\cmsorcid{0000-0003-0228-9760}, R.~Montalvo, K.~Nash, H.~Routray\cmsorcid{0000-0002-9694-4625}, S.~Salur\cmsorcid{0000-0002-4995-9285}, S.~Schnetzer, S.~Somalwar\cmsorcid{0000-0002-8856-7401}, R.~Stone\cmsorcid{0000-0001-6229-695X}, S.A.~Thayil\cmsorcid{0000-0002-1469-0335}, S.~Thomas, J.~Vora\cmsorcid{0000-0001-9325-2175}, H.~Wang\cmsorcid{0000-0002-3027-0752}
\par}
\cmsinstitute{University of Tennessee, Knoxville, Tennessee, USA}
{\tolerance=6000
H.~Acharya, D.~Ally\cmsorcid{0000-0001-6304-5861}, A.G.~Delannoy\cmsorcid{0000-0003-1252-6213}, S.~Fiorendi\cmsorcid{0000-0003-3273-9419}, T.~Holmes\cmsorcid{0000-0002-3959-5174}, N.~Karunarathna\cmsorcid{0000-0002-3412-0508}, L.~Lee\cmsorcid{0000-0002-5590-335X}, E.~Nibigira\cmsorcid{0000-0001-5821-291X}, S.~Spanier\cmsorcid{0000-0002-7049-4646}
\par}
\cmsinstitute{Texas A\&M University, College Station, Texas, USA}
{\tolerance=6000
D.~Aebi\cmsorcid{0000-0001-7124-6911}, M.~Ahmad\cmsorcid{0000-0001-9933-995X}, O.~Bouhali\cmsAuthorMark{97}\cmsorcid{0000-0001-7139-7322}, M.~Dalchenko\cmsorcid{0000-0002-0137-136X}, R.~Eusebi\cmsorcid{0000-0003-3322-6287}, J.~Gilmore\cmsorcid{0000-0001-9911-0143}, T.~Huang\cmsorcid{0000-0002-0793-5664}, T.~Kamon\cmsAuthorMark{98}\cmsorcid{0000-0001-5565-7868}, H.~Kim\cmsorcid{0000-0003-4986-1728}, S.~Luo\cmsorcid{0000-0003-3122-4245}, S.~Malhotra, R.~Mueller\cmsorcid{0000-0002-6723-6689}, D.~Overton\cmsorcid{0009-0009-0648-8151}, D.~Rathjens\cmsorcid{0000-0002-8420-1488}, A.~Safonov\cmsorcid{0000-0001-9497-5471}
\par}
\cmsinstitute{Texas Tech University, Lubbock, Texas, USA}
{\tolerance=6000
N.~Akchurin\cmsorcid{0000-0002-6127-4350}, J.~Damgov\cmsorcid{0000-0003-3863-2567}, V.~Hegde\cmsorcid{0000-0003-4952-2873}, A.~Hussain\cmsorcid{0000-0001-6216-9002}, Y.~Kazhykarim, K.~Lamichhane\cmsorcid{0000-0003-0152-7683}, S.W.~Lee\cmsorcid{0000-0002-3388-8339}, A.~Mankel\cmsorcid{0000-0002-2124-6312}, T.~Mengke, S.~Muthumuni\cmsorcid{0000-0003-0432-6895}, T.~Peltola\cmsorcid{0000-0002-4732-4008}, I.~Volobouev\cmsorcid{0000-0002-2087-6128}, A.~Whitbeck\cmsorcid{0000-0003-4224-5164}
\par}
\cmsinstitute{Vanderbilt University, Nashville, Tennessee, USA}
{\tolerance=6000
E.~Appelt\cmsorcid{0000-0003-3389-4584}, S.~Greene, A.~Gurrola\cmsorcid{0000-0002-2793-4052}, W.~Johns\cmsorcid{0000-0001-5291-8903}, R.~Kunnawalkam~Elayavalli\cmsorcid{0000-0002-9202-1516}, A.~Melo\cmsorcid{0000-0003-3473-8858}, F.~Romeo\cmsorcid{0000-0002-1297-6065}, P.~Sheldon\cmsorcid{0000-0003-1550-5223}, S.~Tuo\cmsorcid{0000-0001-6142-0429}, J.~Velkovska\cmsorcid{0000-0003-1423-5241}, J.~Viinikainen\cmsorcid{0000-0003-2530-4265}
\par}
\cmsinstitute{University of Virginia, Charlottesville, Virginia, USA}
{\tolerance=6000
B.~Cardwell\cmsorcid{0000-0001-5553-0891}, B.~Cox\cmsorcid{0000-0003-3752-4759}, J.~Hakala\cmsorcid{0000-0001-9586-3316}, R.~Hirosky\cmsorcid{0000-0003-0304-6330}, A.~Ledovskoy\cmsorcid{0000-0003-4861-0943}, C.~Neu\cmsorcid{0000-0003-3644-8627}, C.E.~Perez~Lara\cmsorcid{0000-0003-0199-8864}
\par}
\cmsinstitute{Wayne State University, Detroit, Michigan, USA}
{\tolerance=6000
P.E.~Karchin\cmsorcid{0000-0003-1284-3470}
\par}
\cmsinstitute{University of Wisconsin - Madison, Madison, Wisconsin, USA}
{\tolerance=6000
A.~Aravind, S.~Banerjee\cmsorcid{0000-0001-7880-922X}, K.~Black\cmsorcid{0000-0001-7320-5080}, T.~Bose\cmsorcid{0000-0001-8026-5380}, S.~Dasu\cmsorcid{0000-0001-5993-9045}, I.~De~Bruyn\cmsorcid{0000-0003-1704-4360}, P.~Everaerts\cmsorcid{0000-0003-3848-324X}, C.~Galloni, H.~He\cmsorcid{0009-0008-3906-2037}, M.~Herndon\cmsorcid{0000-0003-3043-1090}, A.~Herve\cmsorcid{0000-0002-1959-2363}, C.K.~Koraka\cmsorcid{0000-0002-4548-9992}, A.~Lanaro, R.~Loveless\cmsorcid{0000-0002-2562-4405}, J.~Madhusudanan~Sreekala\cmsorcid{0000-0003-2590-763X}, A.~Mallampalli\cmsorcid{0000-0002-3793-8516}, A.~Mohammadi\cmsorcid{0000-0001-8152-927X}, S.~Mondal, G.~Parida\cmsorcid{0000-0001-9665-4575}, D.~Pinna, A.~Savin, V.~Shang\cmsorcid{0000-0002-1436-6092}, V.~Sharma\cmsorcid{0000-0003-1287-1471}, W.H.~Smith\cmsorcid{0000-0003-3195-0909}, D.~Teague, H.F.~Tsoi\cmsorcid{0000-0002-2550-2184}, W.~Vetens\cmsorcid{0000-0003-1058-1163}, A.~Warden\cmsorcid{0000-0001-7463-7360}
\par}
\cmsinstitute{Authors affiliated with an institute or an international laboratory covered by a cooperation agreement with CERN}
{\tolerance=6000
S.~Afanasiev\cmsorcid{0009-0006-8766-226X}, V.~Andreev\cmsorcid{0000-0002-5492-6920}, Yu.~Andreev\cmsorcid{0000-0002-7397-9665}, T.~Aushev\cmsorcid{0000-0002-6347-7055}, M.~Azarkin\cmsorcid{0000-0002-7448-1447}, A.~Babaev\cmsorcid{0000-0001-8876-3886}, A.~Belyaev\cmsorcid{0000-0003-1692-1173}, V.~Blinov\cmsAuthorMark{99}, E.~Boos\cmsorcid{0000-0002-0193-5073}, V.~Borshch\cmsorcid{0000-0002-5479-1982}, D.~Budkouski\cmsorcid{0000-0002-2029-1007}, V.~Chekhovsky, R.~Chistov\cmsAuthorMark{99}\cmsorcid{0000-0003-1439-8390}, M.~Danilov\cmsAuthorMark{99}\cmsorcid{0000-0001-9227-5164}, A.~Dermenev\cmsorcid{0000-0001-5619-376X}, T.~Dimova\cmsAuthorMark{99}\cmsorcid{0000-0002-9560-0660}, D.~Druzhkin\cmsAuthorMark{100}\cmsorcid{0000-0001-7520-3329}, M.~Dubinin\cmsAuthorMark{90}\cmsorcid{0000-0002-7766-7175}, L.~Dudko\cmsorcid{0000-0002-4462-3192}, A.~Ershov\cmsorcid{0000-0001-5779-142X}, G.~Gavrilov\cmsorcid{0000-0001-9689-7999}, V.~Gavrilov\cmsorcid{0000-0002-9617-2928}, S.~Gninenko\cmsorcid{0000-0001-6495-7619}, V.~Golovtcov\cmsorcid{0000-0002-0595-0297}, N.~Golubev\cmsorcid{0000-0002-9504-7754}, I.~Golutvin\cmsorcid{0009-0007-6508-0215}, I.~Gorbunov\cmsorcid{0000-0003-3777-6606}, A.~Gribushin\cmsorcid{0000-0002-5252-4645}, Y.~Ivanov\cmsorcid{0000-0001-5163-7632}, V.~Kachanov\cmsorcid{0000-0002-3062-010X}, L.~Kardapoltsev\cmsAuthorMark{99}\cmsorcid{0009-0000-3501-9607}, V.~Karjavine\cmsorcid{0000-0002-5326-3854}, A.~Karneyeu\cmsorcid{0000-0001-9983-1004}, V.~Kim\cmsAuthorMark{99}\cmsorcid{0000-0001-7161-2133}, M.~Kirakosyan, D.~Kirpichnikov\cmsorcid{0000-0002-7177-077X}, M.~Kirsanov\cmsorcid{0000-0002-8879-6538}, V.~Klyukhin\cmsorcid{0000-0002-8577-6531}, O.~Kodolova\cmsAuthorMark{101}\cmsorcid{0000-0003-1342-4251}, D.~Konstantinov\cmsorcid{0000-0001-6673-7273}, V.~Korenkov\cmsorcid{0000-0002-2342-7862}, A.~Kozyrev\cmsAuthorMark{99}\cmsorcid{0000-0003-0684-9235}, N.~Krasnikov\cmsorcid{0000-0002-8717-6492}, A.~Lanev\cmsorcid{0000-0001-8244-7321}, P.~Levchenko\cmsAuthorMark{102}\cmsorcid{0000-0003-4913-0538}, N.~Lychkovskaya\cmsorcid{0000-0001-5084-9019}, V.~Makarenko\cmsorcid{0000-0002-8406-8605}, A.~Malakhov\cmsorcid{0000-0001-8569-8409}, V.~Matveev\cmsAuthorMark{99}\cmsorcid{0000-0002-2745-5908}, V.~Murzin\cmsorcid{0000-0002-0554-4627}, A.~Nikitenko\cmsAuthorMark{103}$^{, }$\cmsAuthorMark{101}\cmsorcid{0000-0002-1933-5383}, S.~Obraztsov\cmsorcid{0009-0001-1152-2758}, V.~Oreshkin\cmsorcid{0000-0003-4749-4995}, V.~Palichik\cmsorcid{0009-0008-0356-1061}, V.~Perelygin\cmsorcid{0009-0005-5039-4874}, S.~Petrushanko\cmsorcid{0000-0003-0210-9061}, S.~Polikarpov\cmsAuthorMark{99}\cmsorcid{0000-0001-6839-928X}, V.~Popov, O.~Radchenko\cmsAuthorMark{99}\cmsorcid{0000-0001-7116-9469}, M.~Savina\cmsorcid{0000-0002-9020-7384}, V.~Savrin\cmsorcid{0009-0000-3973-2485}, V.~Shalaev\cmsorcid{0000-0002-2893-6922}, S.~Shmatov\cmsorcid{0000-0001-5354-8350}, S.~Shulha\cmsorcid{0000-0002-4265-928X}, Y.~Skovpen\cmsAuthorMark{99}\cmsorcid{0000-0002-3316-0604}, S.~Slabospitskii\cmsorcid{0000-0001-8178-2494}, V.~Smirnov\cmsorcid{0000-0002-9049-9196}, A.~Snigirev\cmsorcid{0000-0003-2952-6156}, D.~Sosnov\cmsorcid{0000-0002-7452-8380}, V.~Sulimov\cmsorcid{0009-0009-8645-6685}, E.~Tcherniaev\cmsorcid{0000-0002-3685-0635}, A.~Terkulov\cmsorcid{0000-0003-4985-3226}, O.~Teryaev\cmsorcid{0000-0001-7002-9093}, I.~Tlisova\cmsorcid{0000-0003-1552-2015}, A.~Toropin\cmsorcid{0000-0002-2106-4041}, L.~Uvarov\cmsorcid{0000-0002-7602-2527}, A.~Uzunian\cmsorcid{0000-0002-7007-9020}, A.~Vorobyev$^{\textrm{\dag}}$, N.~Voytishin\cmsorcid{0000-0001-6590-6266}, B.S.~Yuldashev\cmsAuthorMark{104}, A.~Zarubin\cmsorcid{0000-0002-1964-6106}, I.~Zhizhin\cmsorcid{0000-0001-6171-9682}, A.~Zhokin\cmsorcid{0000-0001-7178-5907}
\par}
\vskip\cmsinstskip
\dag:~Deceased\\
$^{1}$Also at Yerevan State University, Yerevan, Armenia\\
$^{2}$Also at TU Wien, Vienna, Austria\\
$^{3}$Also at Institute of Basic and Applied Sciences, Faculty of Engineering, Arab Academy for Science, Technology and Maritime Transport, Alexandria, Egypt\\
$^{4}$Also at Ghent University, Ghent, Belgium\\
$^{5}$Also at Universidade Estadual de Campinas, Campinas, Brazil\\
$^{6}$Also at Federal University of Rio Grande do Sul, Porto Alegre, Brazil\\
$^{7}$Also at UFMS, Nova Andradina, Brazil\\
$^{8}$Also at Nanjing Normal University, Nanjing, China\\
$^{9}$Now at Henan Normal University, Xinxiang, China\\
$^{10}$Now at The University of Iowa, Iowa City, Iowa, USA\\
$^{11}$Also at University of Chinese Academy of Sciences, Beijing, China\\
$^{12}$Also at China Center of Advanced Science and Technology, Beijing, China\\
$^{13}$Also at University of Chinese Academy of Sciences, Beijing, China\\
$^{14}$Also at China Spallation Neutron Source, Guangdong, China\\
$^{15}$Also at Universit\'{e} Libre de Bruxelles, Bruxelles, Belgium\\
$^{16}$Also at an institute or an international laboratory covered by a cooperation agreement with CERN\\
$^{17}$Also at Suez University, Suez, Egypt\\
$^{18}$Now at British University in Egypt, Cairo, Egypt\\
$^{19}$Also at Birla Institute of Technology, Mesra, Mesra, India\\
$^{20}$Also at Purdue University, West Lafayette, Indiana, USA\\
$^{21}$Also at Universit\'{e} de Haute Alsace, Mulhouse, France\\
$^{22}$Also at Department of Physics, Tsinghua University, Beijing, China\\
$^{23}$Also at Tbilisi State University, Tbilisi, Georgia\\
$^{24}$Also at The University of the State of Amazonas, Manaus, Brazil\\
$^{25}$Also at Erzincan Binali Yildirim University, Erzincan, Turkey\\
$^{26}$Also at University of Hamburg, Hamburg, Germany\\
$^{27}$Also at RWTH Aachen University, III. Physikalisches Institut A, Aachen, Germany\\
$^{28}$Also at Isfahan University of Technology, Isfahan, Iran\\
$^{29}$Also at Bergische University Wuppertal (BUW), Wuppertal, Germany\\
$^{30}$Also at Brandenburg University of Technology, Cottbus, Germany\\
$^{31}$Also at Forschungszentrum J\"{u}lich, Juelich, Germany\\
$^{32}$Also at CERN, European Organization for Nuclear Research, Geneva, Switzerland\\
$^{33}$Also at Physics Department, Faculty of Science, Assiut University, Assiut, Egypt\\
$^{34}$Also at Wigner Research Centre for Physics, Budapest, Hungary\\
$^{35}$Also at Institute of Physics, University of Debrecen, Debrecen, Hungary\\
$^{36}$Also at Institute of Nuclear Research ATOMKI, Debrecen, Hungary\\
$^{37}$Now at Universitatea Babes-Bolyai - Facultatea de Fizica, Cluj-Napoca, Romania\\
$^{38}$Also at Faculty of Informatics, University of Debrecen, Debrecen, Hungary\\
$^{39}$Also at Punjab Agricultural University, Ludhiana, India\\
$^{40}$Also at University of Hyderabad, Hyderabad, India\\
$^{41}$Also at University of Visva-Bharati, Santiniketan, India\\
$^{42}$Also at Indian Institute of Science (IISc), Bangalore, India\\
$^{43}$Also at IIT Bhubaneswar, Bhubaneswar, India\\
$^{44}$Also at Institute of Physics, Bhubaneswar, India\\
$^{45}$Also at Deutsches Elektronen-Synchrotron, Hamburg, Germany\\
$^{46}$Also at Department of Physics, Isfahan University of Technology, Isfahan, Iran\\
$^{47}$Also at Sharif University of Technology, Tehran, Iran\\
$^{48}$Also at Department of Physics, University of Science and Technology of Mazandaran, Behshahr, Iran\\
$^{49}$Also at Helwan University, Cairo, Egypt\\
$^{50}$Also at Italian National Agency for New Technologies, Energy and Sustainable Economic Development, Bologna, Italy\\
$^{51}$Also at Centro Siciliano di Fisica Nucleare e di Struttura Della Materia, Catania, Italy\\
$^{52}$Also at Universit\`{a} degli Studi Guglielmo Marconi, Roma, Italy\\
$^{53}$Also at Scuola Superiore Meridionale, Universit\`{a} di Napoli 'Federico II', Napoli, Italy\\
$^{54}$Also at Fermi National Accelerator Laboratory, Batavia, Illinois, USA\\
$^{55}$Also at Universit\`{a} di Napoli 'Federico II', Napoli, Italy\\
$^{56}$Also at Ain Shams University, Cairo, Egypt\\
$^{57}$Also at Consiglio Nazionale delle Ricerche - Istituto Officina dei Materiali, Perugia, Italy\\
$^{58}$Also at Riga Technical University, Riga, Latvia\\
$^{59}$Also at Department of Applied Physics, Faculty of Science and Technology, Universiti Kebangsaan Malaysia, Bangi, Malaysia\\
$^{60}$Also at Consejo Nacional de Ciencia y Tecnolog\'{i}a, Mexico City, Mexico\\
$^{61}$Also at Trincomalee Campus, Eastern University, Sri Lanka, Nilaveli, Sri Lanka\\
$^{62}$Also at INFN Sezione di Pavia, Universit\`{a} di Pavia, Pavia, Italy\\
$^{63}$Also at National and Kapodistrian University of Athens, Athens, Greece\\
$^{64}$Also at Ecole Polytechnique F\'{e}d\'{e}rale Lausanne, Lausanne, Switzerland\\
$^{65}$Also at University of Vienna  Faculty of Computer Science, Vienna, Austria\\
$^{66}$Also at Universit\"{a}t Z\"{u}rich, Zurich, Switzerland\\
$^{67}$Also at Stefan Meyer Institute for Subatomic Physics, Vienna, Austria\\
$^{68}$Also at Laboratoire d'Annecy-le-Vieux de Physique des Particules, IN2P3-CNRS, Annecy-le-Vieux, France\\
$^{69}$Also at Near East University, Research Center of Experimental Health Science, Mersin, Turkey\\
$^{70}$Also at Konya Technical University, Konya, Turkey\\
$^{71}$Also at Izmir Bakircay University, Izmir, Turkey\\
$^{72}$Also at Adiyaman University, Adiyaman, Turkey\\
$^{73}$Also at Bozok Universitetesi Rekt\"{o}rl\"{u}g\"{u}, Yozgat, Turkey\\
$^{74}$Also at Marmara University, Istanbul, Turkey\\
$^{75}$Also at Milli Savunma University, Istanbul, Turkey\\
$^{76}$Also at Kafkas University, Kars, Turkey\\
$^{77}$Now at stanbul Okan University, Istanbul, Turkey\\
$^{78}$Also at Hacettepe University, Ankara, Turkey\\
$^{79}$Also at Istanbul University -  Cerrahpasa, Faculty of Engineering, Istanbul, Turkey\\
$^{80}$Also at Yildiz Technical University, Istanbul, Turkey\\
$^{81}$Also at Vrije Universiteit Brussel, Brussel, Belgium\\
$^{82}$Also at School of Physics and Astronomy, University of Southampton, Southampton, United Kingdom\\
$^{83}$Also at University of Bristol, Bristol, United Kingdom\\
$^{84}$Also at IPPP Durham University, Durham, United Kingdom\\
$^{85}$Also at Monash University, Faculty of Science, Clayton, Australia\\
$^{86}$Now at an institute or an international laboratory covered by a cooperation agreement with CERN\\
$^{87}$Also at Universit\`{a} di Torino, Torino, Italy\\
$^{88}$Also at Bethel University, St. Paul, Minnesota, USA\\
$^{89}$Also at Karamano\u {g}lu Mehmetbey University, Karaman, Turkey\\
$^{90}$Also at California Institute of Technology, Pasadena, California, USA\\
$^{91}$Also at United States Naval Academy, Annapolis, Maryland, USA\\
$^{92}$Also at Bingol University, Bingol, Turkey\\
$^{93}$Also at Georgian Technical University, Tbilisi, Georgia\\
$^{94}$Also at Sinop University, Sinop, Turkey\\
$^{95}$Also at Erciyes University, Kayseri, Turkey\\
$^{96}$Also at Horia Hulubei National Institute of Physics and Nuclear Engineering (IFIN-HH), Bucharest, Romania\\
$^{97}$Also at Texas A\&M University at Qatar, Doha, Qatar\\
$^{98}$Also at Kyungpook National University, Daegu, Korea\\
$^{99}$Also at another institute or international laboratory covered by a cooperation agreement with CERN\\
$^{100}$Also at Universiteit Antwerpen, Antwerpen, Belgium\\
$^{101}$Also at Yerevan Physics Institute, Yerevan, Armenia\\
$^{102}$Also at Northeastern University, Boston, Massachusetts, USA\\
$^{103}$Also at Imperial College, London, United Kingdom\\
$^{104}$Also at Institute of Nuclear Physics of the Uzbekistan Academy of Sciences, Tashkent, Uzbekistan\\

